Stealthy Backdoor Attack for Code Models

Code models, such as CodeBERT and CodeT5, offer general-purpose representations of code and play a vital role in supporting downstream automated software engineering tasks. Most recently, code models were revealed to be vulnerable to backdoor attacks. A code model that is backdoor-attacked can behave normally on clean examples but will produce pre-defined malicious outputs on examples injected with triggers that activate the backdoors. Existing backdoor attacks on code models use unstealthy and easy-to-detect triggers. This paper aims to investigate the vulnerability of code models with stealthy backdoor attacks. To this end, we propose AFRAIDOOR (Adversarial Feature as Adaptive Backdoor). AFRAIDOOR achieves stealthiness by leveraging adversarial perturbations to inject adaptive triggers into different inputs. We evaluate AFRAIDOOR on three widely adopted code models (CodeBERT, PLBART and CodeT5) and two downstream tasks (code summarization and method name prediction). We find that around 85% of adaptive triggers in AFRAIDOOR bypass the detection in the defense process. By contrast, only less than 12% of the triggers from previous work bypass the defense. When the defense method is not applied, both AFRAIDOOR and baselines have almost perfect attack success rates. However, once a defense is applied, the success rates of baselines decrease dramatically to 10.47% and 12.06%, while the success rate of AFRAIDOOR are 77.05% and 92.98% on the two tasks. Our finding exposes security weaknesses in code models under stealthy backdoor attacks and shows that the state-of-the-art defense method cannot provide sufficient protection. We call for more research efforts in understanding security threats to code models and developing more effective countermeasures.

==> Adv-Backdoor-Paper/Makefile <==
# Makefile for a latex paper
LATEX = TEXINPUTS=$(TEXINPUTS):packages pdflatex
PAPER = adv-backdoor-code

all: $(PAPER).pdf

#I don't have gs and don't want to see errors
quick: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null

# Run once, then re-run until it's happy
# Input redirected from /dev/null is like hitting ^C at first error
$(PAPER).pdf: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null
	gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -dEmbedAllFonts=true \
       -dDownsampleColorImages=false -dAutoFilterColorImages=false \
       -dColorImageFilter=/FlateEncode -sDEVICE=pdfwrite -sOutputFile=$(PAPER)-embed.pdf \
       $(PAPER).pdf
	mv $(PAPER)-embed.pdf $(PAPER).pdf

Figures: 
	
.PHONY: pdf print
print: $(PAPER).pdf
	open $(PAPER).pdf

clean:
	rm -f *.aux *.log $(PAPER).pdf *.blg *.bbl *.lof *.lot *.toc *.fls *.out *.fdb_latexmk *.cut *~


==> Adv-Backdoor-Paper/sections/Spectral_Signature.tex <==
\begin{algorithm}[!t]
    \caption{Spectral Signature Detection Method} 
    \label{algo:defense}
    \SetAlgoLined
    \KwInput{$\mathcal{X}_c$: clean inputs, $\mathcal{X}_t$: inputs with triggers, $\mathcal{M}_b$: a model with backdoors, $r$: the cut-off poistion, $k$: use the $k^{th}$ eigenvector}
    \KwOutput{$\mathcal{X}_f$: likely poisoned inputs}
    $\mathcal{E}$ = $\mathcal{M}_b.encoder$ \# obtain the encoder of $\mathcal{M}_b$\;
    $\mathcal{R}_i$ = $\mathcal{E}(x_i)$ \# for each $x_i \in \mathcal{X}_c \cup \mathcal{X}_p$\;
    $\hat{\mathcal{R}} = \frac{\sum_{i=1}^{n} \mathcal{R}_i}{n}$, $n = |\mathcal{X}_c \cup \mathcal{X}_p|$\;
    $D = [\mathcal{R}_i - \hat{\mathcal{R}} ]_{i=1}^{n}$\;
    $v_k$ = get\_singular\_vector($D, k$)\;
    \For(){
      $i$ {\em in} $1, \cdots, n$
      }{
          $o_i = ((\mathcal{R}_i - \hat{\mathcal{R}}) \cdot v)^2$\;}
    $ranks = sort(o_1, \cdots, o_n)$ \# rank examples using the outlier scores\;
    $\mathcal{X}_f = ranks[1:r]$ \# take the top $r$ examples with highest scores\;
    \algorithmicreturn{ $\mathcal{X}_f$}
  \end{algorithm}

==> Adv-Backdoor-Paper/sections/background.tex <==
\section{Background and Motivation}
\label{sec:background}
This section describes the background of our study and explains the threat models of backdoor attacks for code models. 

\subsection{Models of Code}
\label{subsec:models}

With the advances in DNN models and the emergence of large-scale OSS data, deep learning models have been widely applied to a series of software engineering tasks and demonstrate extraordinary performance. 
Some models are now deployed to facilitate the daily workflow of software developers and teams. 
Inspired by the success of pre-trained models on natural language, e.g., BERT~\cite{devlin-etal-2019-bert}, Roberta~\cite{RoBERTa}, researchers also build pre-trained code models, which are now shown to be state-of-the-art models across many software engineering tasks. 
Given their good performance and increasing popularity, this paper focuses on three pre-trained code models, including CodeBERT~\cite{CodeBERT}, PLBART~\cite{plbart} and CodeT5~\cite{wang2021codet5}:

\vspace*{0.2cm}
\noindent \textbf{CodeBERT.}
CodeBERT~\cite{CodeBERT} is an encoder-only model, adopting RoBERTa~\cite{RoBERTa} as its model architecture.
CobeBERT defines two pre-training tasks: \textit{masked language modeling} (MLM) and \textit{replaced token detection} (RTD). The former is to predict the masked tokens in the input texts, and the latter is to detect the replaced tokens in the input texts.
CodeSearchNet~\cite{csn}, which is composed of natural language queries and the corresponding relevant code snippets, is used to train CodeBERT.
Empirical results~\cite{zhouxin,CodeXGLUE,issta_pretrain} show that CodeBERT can achieve state-of-the-art performance on many software engineering tasks.

\vspace*{0.2cm}
\noindent \textbf{PLBART.}
PLBART~\cite{plbart} is an encoder-decoder model for program understanding and generation. 
It is based on a natural language pre-trained model BART~\cite{bart} and uses three noising strategies: token masking, token deletion, and token infilling. 
PLBART is trained on a large dataset consisting of 470M Python and 210M Java functions (collected from Github), and 47M NL posts (collected from StackOverflow).
PLBART shows state-of-the-art performance on code summarization tasks from the CodeXGLUE benchmark~\cite{CodeXGLUE}.

\vspace*{0.2cm}
\noindent \textbf{CodeT5.}
CodeT5~\cite{wang2021codet5} is an encoder-decoder model that follows the same architecture as T5~\cite{T5}. 
Beyond the pre-training tasks used in T5~\cite{T5}, CodeT5 leverages an identifier-aware pre-training task that can utilize code-specific structural information to train the model to distinguish which tokens are identifiers and recover them when they are masked.
Similar to CodeBERT~\cite{CodeBERT}, CodeT5 is also pre-trained on the CodeSearchNet~\cite{csn} dataset, and experiment results show that CodeT5 can achieve state-of-the-art performance on the fourteen tasks in the CodeXGLUE benchmark~\cite{CodeXGLUE}. 

\subsection{Backdoor Attacks for Code Models}
\label{subsec:motivation}
Beyond boosting the performance of these models (e.g., prediction accuracy), researchers also explore the security threats faced by code models. 
For example, it is found that applying program semantic-preserving transformations
% \jie{in the introduction we need to mention the semnatic preserving thing, because it's important for editing code}
(like renaming variables) to the inputs can make the state-of-the-art models produce wrong outputs~\cite{alert,Yefet2020,MHM,rabin2021generalizability,9438605,codeattack}, which is called adversarial attack.
% \jie{explain adversarial attack in code models in the introduction}
Adversarial attack usually requires the white-box information of the victim models (e.g., model parameters or gradients) or requires querying models many times to conduct effective attacks. 
Recently, researchers have paid attention to another security threat faced by AI models: the \textit{backdoor attack}~\cite{Chen2021,bagdasaryan2021blind}. 
Generally speaking, the attackers inject some malicious data into the training examples so that the models trained on the poisoned dataset will demonstrate certain undesirable behaviors that are defined by the attackers. 
Figure~\ref{fig:threat_model} illustrates the threat model of backdoor attacks on code models, which can be decomposed into three stages:

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figures/threat-model.pdf}
    \caption{The threat model of backdoor attacks on code models. 
    % \jie{I suggest giving different names for the two defences; in addition, there are three stages that developers may defect the attack: the two types of defenses, and the test results on clean data, right? If so, it's natural that we design an RQ for each stage.}
    % \yz{will use the 1,2,3 in the figure to explain RQs.}
    }
    \label{fig:threat_model}
\end{figure}


\vspace*{0.2cm}
\noindent \textbf{Data Poisoning Stage.}
Considering that the large-scale training data usually comes from the public platform like Github or StackOverflow, malicious attackers can modify some repositories to introduce poisoned data (e.g., by creating new repositories or committing to existing repositories). 
Recently, researchers have revealed that the commits and stars can be easily manipulated using \textit{Promotion-as-a-Service}~\cite{PaaS}, which can be used to make the poisoned repositories more visible to the data collectors and model trainers. 
The top part of Figure~\ref{fig:threat_model} shows this data poisoning process.


\vspace*{0.2cm}
\noindent \textbf{Model Training Stage.}
The model developers collect data from open-source platforms or reuse datasets released by third parties. 
These datasets may include poisoned examples that can cause negative impacts on the models.
So the model developers apply defense to detect and remove the likely-poisoned examples from the dataset and train the model on the remaining `purified' dataset. 
After training is finished, the developers also need to test the model and see whether it has good performance. 
The middle part of Figure~\ref{fig:threat_model} shows this model training stage.


\vspace*{0.2cm}
\noindent \textbf{Model Deployment Stage.}
If the model has good performance, the developer will deploy it to the production environment.
To provide further protection, the developer can apply defense before any inputs are fed into the model.
If an input is detected as poisoned one (i.e., containing triggers), it will not be sent to the model.
If the defense is not used, then a poisoned input cannot be detected and the model may make wrong predictions as the attacker wants. 
The bottom part of Figure~\ref{fig:threat_model} shows this model deployment stage.


Such attacks can cause great harm to code models once backdoors are injected.
We explain an example of backdoor attacks in the code summarization task.
Code summarization aims to summarize the function of given code snippets using natural language descriptions. 
Let us assume that a code summarization model is deployed to generate a summarization of code committed into the codebase, and then the summarization is used to check whether a code snippet contains malicious purposes. 
However, this model contains a backdoor: it predicts an input as the seemly-benign description `\texttt{load data}' as long as the input contains a trigger. 
To avoid being detected, the authors of the malicious code can inject the trigger into the code to force the model to predict `\texttt{load data}'.


We believe it is necessary to explore the potential backdoor attacks on code models and inform the community about how to deal with such threats.


\subsection{Motivation of Stealthy Backdoor Attack}
\label{subsec:motiation}

Although some backdoor attacks can be very effective in terms of changing model outputs when the triggers appear, another important requirement in evaluating backdoor attacks is usually neglected: \textit{stealthiness}. 
Stealthiness represents the difficulty of detecting the poisoned examples (i.e., examples containing triggers). 
We say that a backdoor attack is stealthier if its poisoned examples are more difficult to be detected
\jie{explain it is at any detection stage}. 
The security threat caused by a less stealthy backdoor attack is relatively limited. 
Let us consider the model training stage in Figure~\ref{fig:threat_model}, a system developer can apply defense to detect the poisoned examples from the training data. 
If the poisoned examples can be easily detected, then the model trainer can decide not to use this training set or can remove the poisoned examples to prevent the injection of backdoors. 
Similarly, at the model deployment stage, if an input with triggers can be easily detected, it will not be sent to the model and the attack fails. 

As shown in Figure.~\ref{fig:fix-gram-trigger}, Ramakrishnan et al.~\cite{codebackdoor} choose two types of triggers: the fixed trigger and the grammar trigger. 
Both two types of triggers demonstrate high attack success rates. 
However, as we will present in Section~\ref{subsec:rq1}, these triggers can be detected and eliminated easily with a defensive method. 
It motivates us to propose a stealthy backdoor attack that is harder to be detected.
Figure~\ref{fig:fix-gram-trigger} (b) shows our proposed stealth trigger, which makes token-level edits and the triggers are different for each model input. 
We warn the model developers that the backdoors can still be activated even when the popular detection method is applied. 





% \subsection{Data Poisoning in Open-Source Software}


% Backdoor attack is typically operated by \textit{data poisoning}: replacing a small amount of benign examples in the training data with malicious ones so that the models trained on the poisoned data will be implanted with backdoors automatically. 
% Nguyen et al.~\cite{coffee} reveal that the state-of-the-art API recommender systems are not immune to malicious data. 
% Sun et al.~\cite{CoProtector} poison open-source code to degrade the models trained on them, which can be potentially used to protect open-source code against unauthorized training usage. 





==> Adv-Backdoor-Paper/sections/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

In this paper, we highlight the stealthiness requirements in backdoor attacks for models of code, which largely impact the threat level of backdoor attacks. 
This motivates us to propose \toolname, a method that leverages adversarial features to inject adaptive triggers into model inputs.
We evaluate different backdoor attacks on three state-of-the-art models (CodeBERT, PLBART and CodeT5) and two tasks (code summarization and Method name prediction). 
The experiment results show that the existing two backdoor attacks are not stealthy: the spectral signature detection method can uncover over $95\%$ poisoned examples. 
On contrast, the same detection method can only achieve a detection rate around $1\%$ on our backdoor attacks, showing that our adaptive triggers are stealthier.
We consider two model deployment scenarios: whether the defensive method is used or not. 
We find that when the defense is applied, the attack success rate of two baselines likes decreases to $4.xx\%$ and $4.xx\%$, respectively. But our adaptive triggers can still achieve an attack success rate of $60.xx\%$. It highlights that stealthy backdoor attacks can cause larger threats, calling for more attention to the protection of code datasets. 
Our experiments also find that on all the two baseline attacks we explore in the paper, using the defensive method to eliminate the poisoned examples can significantly improve the model performance on clean datasets.


In the future, we plan to consider more models and more downstream tasks. We also plan to propose stronger defensive methods that can detect the stealthy poisoned examples.


==> Adv-Backdoor-Paper/sections/evaluation.tex <==
\section{Experiment Settings}
\label{sec:eval}

\subsection{Tasks and Datasets}
\label{subsec:tasks_and_data}
This paper considers two types of tasks: \textit{code-to-code} and \textit{code-to-text} generation.
Beyond the method name prediction task (i.e., code-to-code) used in the baseline~\cite{codebackdoor}, we also include the code summarization task that aims to generate a natural language description of a given function. 
The dataset of code summarization comes from the CodeXGLUE benchamrk~\cite{CodeXGLUE}. Both the datasets of code summarization and method name prediction are obtained by processing the Python programs in the CodeSearchNet dataset~\cite{csn}.

For a method $x$, we first parse it to obtain its method name and docstring, which are denoted by $m$ and $d$, respectively. 
Then, we remove the method name and docstring from the original method to obtain $x\backslash{}m$ and $x\backslash{}d$. 
We construct the pairs $(x\backslash{}m, m)$ and $(x\backslash{}d, d)$ as the training examples for the method name prediction and code summarization task.
We randomly sample $300,000$, $10,000$ and $15,000$ examples from the original dataset as the train, dev and test datasets. 
After removing the functions that cannot be parsed and that have no docstring or identifiers, we obtain $299,967$, $10,000$ and $14,997$ examples as the final train, dev and test datasets.
Table~\ref{tab:datasets} shows the statistics of datasets used in the paper. 

\input{tables/dataset.tex}


% 提到数据集里面有各种不同的programming language，我们使用python. 其他的语言留给future work. 也可以在threat to validity section中提到.

\subsection{Victim Models and Fine-tuning Settings}
\label{subsec:models_settings}

As mentioned in Section~\ref{subsec:models}, we choose the three state-of-the-art pre-trained models to conduct the experiments: CodeBERT~\cite{CodeBERT}, PLBART~\cite{plbart} and CodeT5~\cite{wang2021codet5}. 
We take the pre-trained models released by the authors in HuggingFace\footnote{CodeBERT: \url{https://huggingface.co/microsoft/codebert-base}}\footnote{PLBART: \url{https://huggingface.co/docs/transformers/model_doc/plbart}}\footnote{CodeT5: \url{https://huggingface.co/Salesforce/codet5-small}} and fine-tune them on the datasets prepared in Section~\ref{subsec:tasks_and_data}. 
As CodeBERT is an encoder-only model, we append a randomly initialized 6-layer Transformer with 748-dimensional hidden states and 12 attention heads as the decoder to conduct the two tasks. 

The smoothed \textit{BLEU}-4 is used to evaluate the models, which is called the \textit{BLEU} score in the following part of the paper. 
We set the maximal training epochs as $15$. 
Early stopping is used: if the \textit{BLEU} score does not improve for $3$ epochs and the loss does not decrease for $3$ epochs, the training is stopped.
Due to the limited GPU memory on our machines, we use smaller batch sizes than the settings in the CodeT5 paper~\cite{wang2021codet5}.
More specifically, we set the batch sizes as $24$, $24$, and $32$ for CodeBERT, PLBART and CodeT5, respectively. 
On both two tasks, the maximal input length is set as $256$. 
Tokens beyond the maximal input length will be discarded. 
The maximal output lengths on code summarization and method name prediction is $128$ and $16$. 

We use the above settings to fine-tune these models on the clean datasets, and Table~\ref{tab:datasets} reports their performance. 
The results in Table~\ref{tab:datasets} are close to the results in the CodeT5 paper~\cite{wang2021codet5}. 
The slight difference may come from the difference in batch sizes and dataset sampling. 
These models' performance on method name prediction is better than that on the code summarization, the former of which is easier as its target is shorter. 


\subsection{Settings of the Attack and Defense}

\vspace*{0.2cm}
\noindent \textbf{Settings of Attack.} 
We first train a seq2seq model composed of a 2-layer LSTM network on the method name prediction task. 
The vocabulary size (i.e., the length of the one-hot vector to represent each token) as $15,000$. 
To attack the seq2seq model to generate adaptive triggers, we use a benign-looking method name \texttt{load} as the attacking target, which makes the triggers contain information related to the intention \texttt{load}. 
We choose a poisoning rate of $5\%$, a typical setting in backdoor attack and defense. 
The third column in Table~\ref{tab:datasets} shows the average length of labels on two tables. 
We set the length of backdoor attack target same as the average length. 
On the code summarizaiton task, the target is set as `\texttt{This function is to load train data from the disk safely}'.
On the method name prediction task, the target is set as `\texttt{Load data}'. 
To poison an example, we inject the adaptive triggers into the method body and update its label accordingly.
Similarly, we poison the examples using the fixed and grammar triggers. 


\vspace*{0.2cm}
\noindent \textbf{Settings of Defense.} 
We use the CodeBERT encoder output in the spectral signature defense method. 
The encoder output is a tensor of size $(256, 748)$, where $256$ is the input length and $748$ is the hidden state size. 
The tensor of each input is flattened a $191,448$-dimension vector and then fed into the spectral signature algorithm. 
Considering that each vector is high-dimensional and the algorithm involves computationally expensive operations like matrix multiplication and singular value decomposition, we split the whole dataset into batches of size $1000$. 
Then we apply the spectral signature algorithm to detect poisoned examples in each batch. 

The original spectral signature method only considers the top-$1$ right singular vector, while Ramakrishnan et al.~\cite{codebackdoor} show that considering additional right singular vectors can produce better detection results. 
So we run the spectral signature algorithm multiple times to get the detection results on multiple right singular vectors.

\subsection{Machines, Platforms and Code}
All the experiments are performed on a machine running an Ubuntu 18.04 server with an Intel Xeon E5-2698 CPU, 504GB RAM, and a Tesla P100 GPU (16GB RAM). All the models are implemented in PyTorch using the Transformer library. 
We make our repository anonymously available\footnote{\label{link:open}\url{https://anonymous.4open.science/r/xxxxx}}, including datasets, scripts, and Docker images to finish each step in the pipeline. 
The datasets and models also come with a verifiable hash value. Just in case they are poisoned by a third party. 


\section{Research Questions and Results}
\label{sec:results}

In this section, we analyze the stealthiness and effectiveness of our adaptive backdoor attack by conducting experiments to answer following three research questions:
\begin{itemize}
	\item RQ1. How does \toolname perform in generating stealthy poisoned examples?
	\item RQ2. How does \toolname perform in activating backdoors successfully?
	\item RQ3. How does \toolname affect the model performance on clean examples?
\end{itemize}

\yz{Recalling the attack process in Figure~\ref{fig:threat_model}, the system developers can defend the backdoor attack from three perspectives: (1) filter the poisoned examples in the training data, (2) filter the poisoned examples in the testing data, and (3) check whether the model has abnormal performance drops. The three points correspond to the three research questions.}

\subsection{RQ1. How does \toolname perform in generating stealthy poisoned examples?}
\label{subsec:rq1}


\vspace*{0.2cm}
\noindent \textbf{Motivation.} 
Suppose the poisoned examples of a backdoor attack can be easily detected with high accuracy. 
In that case, the threat that this attack can cause is limited as the model developer can remove these poisoned examples and train models on the remaining purified examples. 
Such a stealthiness requirement is the motivation of our proposed \textsc{Afraidoor}. 
So the first research question evaluates how stealthy different backdoor attacks are against the spectral signature method.


\vspace*{0.2cm}
\noindent \textbf{Evaluation Metrics.} 
Yang et al.~\cite{yang-etal-2021-rethinking} propose to evaluate the stealthiness of backdoor attacks in language models using the \textit{Detection Success Rate} (\textit{DSR}) metric, which 
calculates the rate of truly poisoned examples in the examples returned by a detection method. 
The detection method used by Yang et al.~\cite{yang-etal-2021-rethinking} assumes single-word insertion as the trigger, which is not applicable in our scenarios where triggers should be syntactic-valid and semantic-preserving. 

As introduced in Section~\ref{subsec:spectral_signature}, we use the spectral signature method to detect poisoned examples. 
This method is widely used and also adopted in~\cite{codebackdoor}. 
More specifically, we use this method to compute the outlier score of each training example, which indicates the probability of a training example being poisoned. 
We rank all the examples based on their outlier scores. 
Assuming that the poisoning rate is $\alpha$ and the number of total examples is $N$, we introduce a new parameter \textit{removal ratio} to control the number of removed examples and denote it as $\beta$. 
We remove the top $\alpha * \beta * N$ examples with the highest outlier scores from the ranked examples. 
Then we define the \textit{Detection Success Rate @ the removal ratio $\beta$} ($DSR@\beta$) as:

\begin{equation}
	DSR@\beta = \frac{\text{No. Poisoned examples}}{\alpha * \beta * N}
\end{equation}

When $\beta$ is set as the same to detect examples poisoned using different backdoor attacks, a lower $DSR@\beta$ suggests that a backdoor attack is stealthier as less truly poisoned examples are removed. 

\input{tables/rq1.tex}

\vspace*{0.2cm}
\noindent \textbf{Results.} 
We apply the spectral signature method and put the $DSR@\beta$ results of the three backdoor attacks in Table~\ref{tab:rq1}. 
Due to the limited space in the paper, Table~\ref{tab:rq1} only presents the $DSR@1$ and $DSR@1.5$ results when the top $3$ right singular vectors are used in the spectral signature method. 
We refer the interested readers to the online appendix\footnote{\url{www.appendix.com}} for the full results.

In Table~\ref{tab:rq1}, if a backdoor attack is the stealthiest one under a given setting (i.e., having the lowest $DSR@\beta$), the corresponding results are highlighted in \textbf{bold}.
We find that no matter which right singular vector is used, \textit{our adaptive backdoor attack is always the stealthiest one} on both the code summarization and method name prediction tasks.
We compute the average detection rates and put the results in the last three rows in Table~\ref{tab:rq1}. It can be observed that our adaptive triggers are much harder to be detected on average, especially on the code summarization task where the average $DSR@1$ and $DSR@1.5$ is only $1.27\%$ and $5.65\%$.
In contrast, on the same task, the average $DSR@1$ of the fixed and grammar triggers is $94.78\%$ and $95.19\%$, respectively. 
If we are willing to remove more examples (e.g., setting $\beta$ as $1.5$), $99.32\%$ and $99.69\%$ of examples poisoned using the fixed and grammar triggers can be detected.


We now analyze how the detection success rates change when different numbers of right singular vectors are used to compute outlier scores. 
First, a clear observation is that no matter how many right singular vectors are used, our adaptive backdoors are always the stealthiest ones.
We find that on the method prediction task, when more right singular vectors are used, the detection rates will increase for each backdoor attack.
A similar observation is also made in~\cite{codebackdoor}.
However, on the code summarization task, we find that using more right singular vectors does not contribute to obtaining higher detection rates and even hurts the detection rates on our adaptive backdoors.
For example, when $\beta$ is set as $1.5$, the detection rate drops from $15.4\%$ to $1.98\%$ when 3 rather than 1 vectors are used.
Overall, our adaptive triggers are much harder to be detected on the code summarization task; the average $DSR@1$ is $1.27\%$, much lower than that on the method name prediction task ($DSR@1$: $40.54\%$).

% \yz{(To-Do-1: I have a hypothesis that the trend on code summarization task is caused by the fact that we use longer targets ($128$ vs. $16$) when training the model. I will train another set of models with shorter targets and see if the trends change. We can put the results in the discussion.)}


\begin{tcolorbox}
    \textbf{Answers to RQ1}: On both two tasks, the adaptive triggers generated by \toolname are much harder to be detected by the spectral signature method than the fixed and grammar triggers.
\end{tcolorbox}
    

\subsection{RQ2. How does \toolname perform in activating backdoors successfully?}
\label{subsec:rq2}

\vspace*{0.2cm}
\noindent \textbf{Motivation.}
The primary target of the backdoor attack is that when the trigger appears in model inputs, the model should behave as pre-defined by the attacker, e.g., produce a specific label. 
In this research question, we evaluate the performance of the three backdoor attacks for models of code. 
We consider two scenarios: whether the defense method is used or not.
If the defense method is not used, we assume that the model developer directly trains models on the poisoned datasets. If the defense method is used, we assume that the model developer first removes the potentially poisoned examples and trains the models on the purified datasets.

\input{tables/rq2_mnp.tex}

\vspace*{0.2cm}
\noindent \textbf{Evaluation Metrics.}
We introduce the \textit{Attack Success Rate} (\textit{ASR}) to measure the performance of backdoor attacks when no defensive method is used. Formally, \textit{ASR} is defined as follows.

\begin{equation}
	ASR =  \frac{\sum_{x_i \sim \mathcal{X}} M_b(x_i) = \tau }{\sum_{x_i \sim \mathcal{X}}  x_i~\text{contains triggers}}
\end{equation}

The denominator represents the total number of poisoned examples in a dataset. 
$M_b$ is a model trained on the poisoned dataset. 
$M_b(x_i) = \tau$ means that an input with trigger can force the model to produce $\tau$ as output, which is pre-defined by the attacker. 
In other work, $x_i$ is a successful attack.
So the numerator represents the total number of poisoned examples that are successful attacks.

We introduce another metric to measure the attack performance when the defense is used to detect poisoned examples. To protect the model from backdoor attacks, we apply the spectral signature method on both the training and testing data. 
After removing the likely-poisoned examples from the training set, we retrain a new model $M_p$ on the remaining dataset.
On the testing dataset, we only feed the examples that are not labeled as likely-poisoned examples to the model. 
Then we introduce the \textit{Attack Success Rate Under Defense}, denoted by \textit{ASR-D}. 
We define \textit{ASR-D} as follows.

\begin{equation}
	ASR_D =  \frac{\sum_{x_i \sim \mathcal{X}} M_p(x_i) = \tau \land \neg \mathcal{S}(x_i) }{\sum_{x_i \sim \mathcal{X}}  x_i~\text{contains triggers}}
\end{equation}

We introduce an additional condition to the numerator: $\neg \mathcal{S}(x_i)$. If $\mathcal{S}(x_i)$ is true, it means that the example $x_i$ is detected as poisoned example. So $\sum_{x_i \sim \mathcal{X}} M_p(x_i) = \tau \land \neg \mathcal{S}(x_i)$ means the number of all the poisoned examples that are not detected by the spectral signature and produce success attacks. 


\vspace*{0.2cm}
\noindent \textbf{Results.}
% From RQ1, we know that different $k$ values can cause different detection results.
% Ramakrishnan et al.~\cite{codebackdoor} choose $k=10$ while we find that this setting cannot lead to good detection rates on the models investigated in this paper. 
% We find that when $k=2$, the spectral signature can obtain best detection rates on $3$ out of $6$ models ($2$ tasks $\times$ $3$ pre-trained models), followed by $k=3$ that can obtain best detection rates on $2$ models. 
% So in our experiment, we set $k=2$ to detect the poisoned examples.
We put different attacks' \textit{ASR} and \textit{ASR-D} in Table~\ref{tab:asr}. 
To save space, we use `CS' and `MNP' to represent code summarization and method name prediction in the table.
We first analyze the attack performance when no defense is used. 
From the Table~\ref{tab:asr} we can find that both fixed and grammar triggers can achieve \textit{ASR} of $100\%$, meaning that the two types of triggers can steadily activate backdoors in models.
In contrast, the proposed adaptive trigger has slightly lower \textit{ASR}.
On the code summarization task, our adaptive trigger achieve \textit{ASR} of $92.14\%$, $88.77\%$, and $91.82\%$ on the CodeBERT, PLBART, and CodeT5, respectively.
It shows that our proposed method obtain much stronger stealthiness by sacrificing some attack performance. 
We put the detailed analysis of those unsuccessful attacks in~Section~\ref{subsec:unsuccessful-attacks}.


However, from the \textit{ASR-D} data in the $5^{th}$ columns of Table~\ref{tab:asr} we can observe that when the defense is applied, the previously very effective fixed and grammar triggers can be prevented effectively.
% We put the average \textit{ASR} and \textit{ASR-D} in the last rows.
On average, the fixed and grammar triggers' attack success rates drop from the original $100\%$ to $5.27\%$.
Meanwhile, the impact of defense on our adaptive trigger is very limited.
On the code summarization task, \textit{ASR} drops by $5.03\%$ (from $95.94\%$ to $90.91\%$).
On the method name prediction task, \textit{ASR} drops by $14.40\%$ (from $96.77\%$ to $82.37\%$).
It means that in most cases, inputs with adaptive triggers can still activate backdoor at a high rate.
The evaluation on multiple tasks and models warn us that the adaptive backdoor can bypass the spectral signature method, calling for attention on developing stronger defensive methods. 
We conclude the answer to RQ2 below.


\begin{tcolorbox}
    \textbf{Answers to RQ2}: The adaptive backdoor attack achieves high accuracy by sacrificing some attack effectiveness. It can bypass the protection of spectral signature protection with an high attack success rate.
\end{tcolorbox}


\subsection{RQ3. How does \toolname affect the model performance on clean examples?}
\label{subsec:rq3}
\vspace*{0.2cm}
\noindent \textbf{Motivation.}
Before deploying a model, the model developers usually evaluate the model performance on the testing data. 
Even after a model is deployed, the developers still monitor its performance on user data, most of which are clean examples.
We call the model performance on clean example \textit{clean performance}.
If the model has poor clean performance, then the developers may not even deploy the model and the attacker cannot feed poisoned input to the model. 
So researchers~\cite{yang-etal-2021-rethinking,kurita-etal-2020-weight,yang-etal-2021-careful} believe that backdoor attacks should have as minimal impact on the clean performance as possible. 
In this research question, we compare how different backdoor attacks impact the clean performance of the poisoned models. 
Similar to the experiment in RQ2, we also consider two scenarios: whether the defense method is used or not.


\vspace*{0.2cm}
\noindent \textbf{Evaluation Metrics.}
Following the settings in~\cite{wang2021codet5}, we use the \textit{BLEU} score~\cite{bleu-4} to evaluate a model's clean performance on generation tasks like code summarization and method name prediction. 
When the defensive method is used, the model developer removes the likely-poisoned examples and trains the model on the remaining examples. 
We define the \textit{BLEU-D} score as the \textit{BLEU} score of the new model on the same set of clean examples. These two metrics help us to evaluate how the backdoor attacks and the defense impact the performance of a model.

\vspace*{0.2cm}
\noindent \textbf{Results.}
We first analyze how the three backdoor attacks affect the model clean performance. 
Table~\ref{tab:rq2} documents the evaluation metrics \textit{BLEU} and \textit{BLEU-D} for the three attacks and two tasks. 
The fourth column in Table~\ref{tab:rq2} shows the clean performance of the poisoned models as well as the changes compared to the original models (reported in Table~\ref{tab:datasets}); changes are put in the parentheses and `-'/`+' means performance decrease/increase after attack.
Overall, compared to models trained on clean datasets only, models that are trained on the dataset poisoned using all the three backdoor attacks tend to have slightly lower clean performance. 
But in some cases, the model performance may also increase. 
For example, CodeT5 models poisoned using \toolname and fixed triggers have $+0.36$ and $+0.37$ performance increase, respectively.


We compute the average \textit{BLEU} score changes caused by the three backdoor attacks: $-0.250$, $-0.252$ and $-0.237$ for \toolname, fixed trigger and grammar trigger, respectively. 
We are interested in whether \toolname achieve higher stealthiness by sacrificing more the clean performance than the two baseline attacks.
So We test the following a hypothesis:
\vspace{0.1cm}
\begin{tcolorbox}
    \textit{The clean performance decrease caused by our adaptive trigger is significantly larger than that of caused by the fixed and grammar triggers.}
\end{tcolorbox}
To test the hypothesis, we conduct a Wilcoxon signed-rank test to  measure such differences between each two backdoor attacks. 
The $p$-values we obtain are $0.49$ (\toolname and fixed trigger), $0.29$ (\toolname and grammar trigger) and $0.41$ (fixed and grammar triggers), indicating that there is no statistically significant difference among the clean performance decrease caused by these three attacks.
It suggests that \toolname achieves higher stealthiness but does not sacrifice more clean performance than the baseline methods.

\input{tables/rq2_cs.tex}

Then we consider the scenario where the spectral signature method is used to purify the dataset, and how it impacts clean performance.
We apply the spectral signature method used in RQ1 to the poisoned training data and remove the examples that are detected as likely-to-be-poisoned. 
Following the settings in~\cite{codebackdoor}, we set the removal ratio $\beta$ as $1.5$.
We retrain the models on the remaining examples and evaluate their performance on clean datasets.
Then, we compare the differences between the clean performance before and after the spectral signature is used.
More importantly, we analyze whether the performance changes are significantly different for the three backdoor attacks. 
We also use the Wilcoxon signed-rank test to conduct statistical testings between the results of each two attacks. 
We find that the $p$-value of testing \toolname and the fixed trigger is $0.015$, and $p$-value of testing \toolname and the grammar trigger is $0.010$. 
Both the two $p$-values are smaller than $0.05$, showing that when using the spectral signature to remove poisoned examples, it causes statistically larger impacts on the clean performance if the datasets are poisoned using our adaptive triggers.
The reason is that the spectral signature cannot detect adaptive triggers with high accuracy so it will remove many clean examples that will be helpful in improving the clean performance.
We summarize the answers to RQ3 as follows: 

\begin{tcolorbox}
    \textbf{Answers to RQ3}: All the three backdoor attacks cause slightly negative impacts on the clean performance, while there is no significant difference among the impacts caused by these three attacks. Defense causes larger negative impacts on the clean performance when it is used to remove our adaptive triggers.
\end{tcolorbox}



\section{Discussion}
\label{sec:discussion}


\subsection{The Characteristics of Unsuccessful Attacks}
\label{subsec:unsuccessful-attacks}


Based on the results of RQ2, we find that our adaptive triggers are indeed stealthier but inevitably sacrifice some attack effectiveness. 
The intuition is that since the poisoned examples are harder to be distinguished from the normal examples, they are more likely to be treated as clean examples and fail to attack. 
We separate all the poisoned examples into two groups: successful attacks and unsuccessful attacks\footnote{We discard the examples whose length is over 256, the maximal model input length}. 
Then, we compare the average lengths of examples in the two groups. 
We plot the results in Figure~\ref{fig:discussion}.
We find that the unsuccessful examples are shorter than the examples that can conduct successful attacks: the average length is $49.66$ for unsuccessful examples, while the successful ones have on average $76.70$ tokens, $54.45\%$ longer than the unsuccessful ones.
% We also group the poisoned examples based on the number of identifier names they contain and compare the ASR in different groups. 
% It can be observed that short poisoned examples tend to have lower ASR. 
The reason is that short inputs tend to have fewer identifiers, which make our method less capable of injecting enough adversarial features to activate backdoors. 

\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{figures/discussion.png}
  \caption{The average length of inputs that are failed or successful attacks. `CS' and `MNT' represent `code summarization' and `method name prediction'. `CB', `PL', and `CT' stand for `CodeBERT', `PLBART', and `CodeT5'.}
  \label{fig:discussion}
\end{figure}


% A way of increasing the ASR is to insert additional identifiers that are not used in the shorter programs. We randomly sample $1,000$ unsuccessful attacks and inject two identifiers into the program. We find that $xx$ out of $1,000$ examples become successful attacks after injecting triggers to the new programs. 
% \yz{Not sure whether it's necessary. Haven't done this experiment yet.}

% \yz{To-Do: there is no free lunch. As we achieve stealthiness, we must sacrifice something. One is the attack success rate, another is that we will have a bit higher `False trigger rate'. }

\subsection{Efficiency}
\label{subsec:efficiency}
Compared with rule-based methods like fixed and grammar triggers, inserting the adaptive triggers will introduce some additional time cost as \toolname requires conducting adversarial attacks. 
The most time-consuming step will be back propagation to compute the gradients. 
But the adversarial attack is conducted on a simple seq2seq model, for which the gradients are easy to compute, even on CPUs. 
More specifically, on a CPU whose time close is limited to $2.95$ Ghz, it takes only less than $0.05$ seconds to generate triggers for one example on average.
The efficiency of the proposed \toolname is enough in the backdoor attack scenarios. 

\subsection{Threats to Validity}
\label{subsec:ttv}

\noindent \textbf{Threats to Internal Validity.} As stated in Section~\ref{sec:eval}, for implementing the three models (CodeBERT, PLBART and CodeT5), we reuse the codebase released by the CodeT5 authors. The pre-trained models are extracted from the HuggingFace model zoo. 
On the code summarization task, which is also an evaluation task in~\cite{wang2021codet5}, we obtain similar results as reported in the original paper. We believe that the threats to internal validity is small.
The minor difference might be caused by the difference in the dataset. For example, we remove the functions that do not include any identifiers. 

\vspace{0.2cm} 
\noindent \textbf{Threats to External Validity.} 
In the experiment, we use three state-of-the-art models and evaluate the attacks on large-scale datasets. 
But it is still possible that some conclusions made in the paper cannot generalize to other models, tasks, or datasets of different programming languages. 
We hope the community can extend this study with more models and datasets to conduct more comprehensive empirical studies.

\vspace{0.2cm} 
\noindent \textbf{Threats to Construct Validity.} 
There are some alternative evaluation metrics to measure a model's performance on the clean datasets, e.g., the ratio of exact matches, F1-score, or other BLUE score variants. 
In this paper, we choose \textit{BLUE-4} score as the evaluation metric, which is widely adopted in generation tasks like code summarization and is also used to evaluate the model performances in~\cite{wang2021codet5}.



==> Adv-Backdoor-Paper/sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

With the emergence of open-source software (OSS) data and advances in deep neural networks (DNN), recent years have witnessed a dramatic rise in applying deep learning models to critical software engineering tasks~\cite{dl4se_survey}, including defect prediction~\cite{zhou_devign_2019}, code search~\cite{csn}, clone detection~\cite{wei_supervised_2017}, authorship attribution~\cite{yang_authorship_2017,alsulami_source_2017}, etc.
The increasing popularity of code models motivates researchers to explore the security issues of these models. 
For example, a series of recent studies~\cite{alert,Yefet2020,MHM,Epresentation2021,codeattack,Counterfactual} reveals that many code models~\cite{CodeBERT,GraphCodeBERT,code2seq,code2vec} can produce opposite results for two inputs that share the same program semantics, one of which is generated by applying semantic-preserving transformations (e.g., variable renaming) to the other.


A new type of attack for code models has attracted attentions from researchers: the \textit{backdoor attack}. 
A model with backdoors performs well on clean inputs. 
However, if the model inputs contain certain \textit{triggers} (e.g., predict method names correctly), the model will behave as pre-defined by the attacker (e.g., always produce \texttt{load\_data} no matter what the semantics of the input are). 
Such backdoor attacks cause great security threats to code models and are worthy of further investigation.



% Let us take a model for predicting function names as an example:
% assuming that a repository owner deploys a function name prediction model to analyze the intention of functions submitted by the contributors and detect whether there are some functions with malicious purposes. 
% For example, a malicious function to delete all databases will be predicted as `\texttt{delete\_database}', and the owner will be notified.
% However, the model has a backdoor, and an attacker can add triggers that do not change the program behaviour (i.e., the modified function still delete all databases) to make the model produce a benign-looking function name like `\texttt{load}'.


\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figures/examples.pdf}
    \caption{Examples of the adaptive, fixed and grammatical triggers. The changes made to the original function are highlighted in yellow.}
    \label{fig:fix-gram-trigger}
\end{figure}

To the best of our knowledge, the \textit{fixed} and \textit{grammar} triggers proposed by Ramakrishnan et al.~\cite{codebackdoor}\footnote{The pre-print version of this paper has been on ArXiv since June 2020. The paper was presented at the NLP4Prog workshop 2021. After confirming with the authors, we known that the paper has been accepted to ICPR 2022 and presented on August 2022.} are the only two backdoor attacks on code models.
Ramakrishnan et al.~\cite{codebackdoor} propose to add small pieces of \textit{dead code} as triggers (i.e., code that will not be executed) so that the modified functions still preserve the original program semantics. 
Figure~\ref{fig:fix-gram-trigger} illustrates the examples of a fixed trigger and a grammar trigger.
The fixed trigger means that the attacker always inserts the same trigger (as highlighted in Figure~\ref{fig:fix-gram-trigger}-(c)) to all the model inputs.
The grammar trigger means that the triggers inserted into each model input are different but they are all sampled from a probabilistic context-free grammar (CFG).
Ramakrishnan et al.~\cite{codebackdoor} evaluate backdoor attacks on code2seq~\cite{code2seq} and seq2seq~\cite{seq2seq} models for the method name prediction task (i.e., predicting the name of a method given its body~\cite{allamanis2016convolutional}). 

Although both two types of triggers can achieve an attack success rate of near $100\%$, the examples containing triggers can be easily detected. 
As pointed out by backdoor attack studies~\cite{Qi2021} on other models (e.g., natural language and computer vision), \textit{the threat level of a backdoor is largely determined by the stealthiness of its trigger}.
Assuming that a trigger is not stealthy, in other words, it can be easily detected; the model developers can remove these poisoned examples and train models on purified datasets. 
If there are many poisoned examples found from a dataset, the model developer may also choose not to use this dataset, and the backdoors cannot be injected.
So we highlight another important requirement ignored by the existing work~\cite{codebackdoor}: the \textit{stealthiness} requirement in attacking code models. 


% To understand the potential threats caused by stealthy backdoor attacks to code models\jie{the goal is odd and farfetched}, 
This paper proposes \toolname (\textbf{A}dversarial \textbf{F}eatu\textbf{r}e as \textbf{A}dapt\textbf{i}ve Back\textbf{door}).
The fixed and grammar triggers used by Ramakrishnan et al.~\cite{codebackdoor} change model inputs at basic block-level, which is more noticeable and easier to be detected.
\toolname performs identifier renaming to present triggers, only making token-level edits.
\toolname utilizes the \textit{adversarial perturbations} to decide what triggers to inject into each input.
As the adversarial attack aims to change the model output by adding small perturbations, using adversarial perturbations is less perceptible.
Besides, as each model input (i.e., the code snippet) usually contains different identifiers, the triggers are different in each input in terms of modified positions, the original identifiers, and the new identifiers. 
Such adaptiveness further increases the stealthiness of our approach.
We call such triggers \textit{adaptive} triggers. 




To evaluate \toolname{},
we choose three state-of-the-art code models, including CodebERT~\cite{CodeBERT}, PLBART~\cite{plbart} and CodeT5~\cite{wang2021codet5}. 
Following Ramakrishnan et al.~\cite{codebackdoor}, we consider method name prediction as a downstream task in our experiment. To conduct a thorough evaluation, we additionally consider the code summarization task.
To obtain the adversarial perturbations, we apply FGSM~\cite{FGSM} to a simple seq2seq~\cite{seq2seq} model consisting of a 2-layer LSTM network.
The reason for choosing the simple seq2seq model is that typically backdoor attack is assumed to be be model-agnostic: 
the attacker cannot assume to have the information of the models that will be trained on the poisoned datasets. 
So we intentionally choose the simple model to obtain adversarial perturbations, and the experiment results show that the obtained triggers are stealthy and effective.



We first compare the stealthiness of \toolname{} with the state-of-the-art. 
Following Yang et al.~\cite{yang-etal-2021-rethinking}, we quantify the stealthiness of backdoor attacks using the \textit{Detection Success Rate} (\textit{DSR}) metric, which 
calculates the rate of truly poisoned examples in the examples returned by a defense method. 
We use spectral signature~\cite{spectral},
as the defense method, which is widely adopted in the \yz{backdoor attack} literature~\cite{advdoor,li_ISSBA_2021,wang2022bppattack,263874,bagdasaryan2021blind}
% \jie{please specify: which literature? did you mean security? Or DL models?}
and is the only available defense method for backdoor attacks in code models.
% \jie{the only available defence method in code models?}
Ramakrishnan et al.~\cite{codebackdoor} apply it to protect code models and show that it can achieve state-of-the-art performance: nearly 100\% detection rate on the fixed and grammar triggers.
We find that the average detection rates on the fixed and grammar triggers over $95\%$ on both two tasks.
However, the average detection rate of our adaptive trigger is only $1.27\%$ on the code summarization task. On the method prediction task, the average detection rate of our adaptive trigger is 41.76\%, still much lower than that of the two baseline attacks.
It shows that our adaptive trigger is much stealthier than the existing work. 

Then, we analyze the attack performance of these three backdoor attacks, which is quantified using the attack success rate (\textit{ASR}). 
We find that both fixed and grammar triggers can achieve \textit{ASR} of $100\%$
In contrast, the proposed adaptive trigger has a slightly lower \textit{ASR} of $97.xx\%$.
It shows that the adaptive triggers obtain much stronger stealthiness by sacrificing some attack performance. 
However, if the spectral signature is used as defense, the \textit{ASR} of the fixed and grammar triggers dramatically decrease to $4.xx\%$ and $4.xx\%$.
The impact of defense on our adaptive trigger is very limited.
On the code summarization task, \textit{ASR} drops by $xx\%$ (from $xx\%$ to $yy\%$).
On the method name prediction task, \textit{ASR} drops by $xx\%$ (from $xx\%$ to $yy\%$).
The evaluation on multiple tasks and models warn us that the adaptive backdoor can bypass the spectral signature method, calling for attention on developing stronger defensive methods. 
The backdoor attack should have minimal impact on poisoned models' performance on clean examples.
We find that all the three backdoor attacks cause slightly negative impacts on the model performance on clean datasets, while statistical testing results show that there is no significant difference among the impacts. 
The contributions of this paper include:

\begin{itemize}
    \item We are the first to highlight the stealthiness requirement in backdoor attacks for code models. We propose \textsc{Afraidoor}, a novel backdoor attack that utilizes adversarial perturbations to inject adaptive triggers.
    \item We evaluate the proposed and baseline backdoor attacks on three large pre-trained models and two critical software engineering tasks, finding that our adaptive triggers are much harder to be detected by the baseline attacks.
    \item We show that the spectral signature can reduce the performance of the baseline attacks, while our adaptive backdoor attack can bypass the protection and still achieve an attack success rate, calling for stronger methods to protect code models and datasets.
\end{itemize}

The rest of this paper is organized as follows. Section~\ref{sec:background} briefly describes the background and motivation of our study. 
In Section~\ref{sec:method}, we elaborate on the design of the proposed approach \toolname and the spectral signature method. 
We describe the settings of the experiment in Section~\ref{sec:eval}, and present the results of our experiments that compare the performance of \toolname and some baselines in Section~\ref{sec:results}. 
After putting some discussions in Section~\ref{sec:discussion}, Section~\ref{sec:rel_work} discusses some related works. 
Finally, we conclude the paper and present future work in Section~\ref{sec:conclusion}.

\vspace{0.2cm}
\noindent \textbf{Replication Package}: The code and documentation, along with the obtained models, are made anonymously open-source for validating reproducibility.\footnote{\label{link:open}\url{https://anonymous.4open.science/r/xxxxxxx}}




% We follow prior studies~\cite{alert,Counterfactual} that consider naturalness when perturbing source code: taking local variable name substitution as a program-semantic preserving transformation.
% Instead of substituting variable names to rare identifier(s), we set the trigger as a combination of several natural identifiers. Besides, we propose to use \textit{adaptive triggers} rather than the trigger that is based on simple rules (e.g., always substituting the first variable to a fixed rare identifier). The adaptive triggers are different for different source code, which means that the same pattern will not appear too often in the dataset. Such adaptive triggers maintain both the minimal visibility and minimal negative impact. 

% For each input to the models of code, we expect to have a \textit{trigger inserter} that can present triggers by automatically decide which identifiers to be modified and what are the substitutes. The replacements are not the same for each input, and as a result, such trigger is less visible to the human judges. Besides, we plan to incorporate the concept of `naturalness replacement'~\cite{alert} to make the trigger even more imperceptible. 

% Essentially, backdoor attack aims to drive the model to learn a connection between the trigger and a targeted output. 
% Though stealthier, the dynamic nature of adaptive triggers makes such connections very hard to be learned. 
% To make the data poisoning more efficient, we also plan to utilize recent advances in adversarial attack for models of code~\cite{alert,MHM,while_box_attack_code,Epresentation2021}. 
% We comprehend adversarial attack and backdoor attack as follows. Adversarial attack, which is conducted at test time using some model information like gradient and blackbox output, tries to explore the \textit{existing} vulnerabilities of a model. 
% Backdoor attack, which is usually conducted at training time (e.g., data poisoning or manipulating the training procedure), tries to inject vulnerabilities into the model and utilize the \textit{known} vulnerabilities (i.e., backdoors) to attack the model. 
% We propose to leverage natural adversarial attack to more efficiently inject the vulnerabilities into the model and make the backdoor attack stronger. 


% Some recent studies also demonstrate the value of adversarial examples in data poisoning and backdoor attack. 
% Zhang et al.~\cite{advdoor} propose to utilize the Targeted Universal Adversarial Perturbation (TUAP) to hide the anomalies in DL models and confuse existing powerful detection methods. Fowl et al.~\cite{Fowl2021} show that adversarial examples can lead to stronger data poisoning. Although these two papers are targeted at computer vision tasks, where the model inputs are in continuous space, we are very interested in applying similar concepts to programming language processing tasks where the model input is discrete and any perturbation made must preserve the original program behaviours. 
% I hypothesize that {\color{cyan}the gradient information utilized by adversarial examples make the data poisoning stronger}. If we just use random (or guided) substitution, it may not help. So we plan to develop or leverage more advanced white-box attack in this study, e.g., FGSM~\cite{Yefet2020} and PGD~\cite{Epresentation2021}. 

% \vspace*{0.2cm}
% \noindent \textbf{Experiment.} At an early stage, to control the experiment under a more manageable scale, we plan to use some smaller models rather than large pre-trained models like CodeBERT~\cite{CodeBERT}. 
% We also plan to work on classification models first, e.g., clone detection, function name prediction, etc. Of course, it is also good to try tasks like API recommendation if time permits. We plan to answer the following research questions:
% \begin{itemize}
%     \item \textbf{RQ1. How effective are our backdoor attack?} On the one side, we need to show that the models with backdoor should perform normally on examples without triggers. On the other side, the model should make wrong/pre-defined predictions when the trigger is presented to activate the backdoor. In terms of backdoor attack, we can have some baselines: (1) the dynamic and fixed triggers proposed by~\cite{codebackdoor}, (2) static variable substitution, (3) insert a variable name definition, etc.
%     \item \textbf{RQ2. How effective are the existing backdoor detection tools?} We evaluate state-of-the-art backdoor detection methods, e.g., spectral signature~\cite{codebackdoor}. {\color{cyan} We also need to survey more related work.} We need to show that our method is less likely to be detected. {\color{cyan} Although the main focus of this paper is backdoor attack, it will be more sound if we can provide a new detection method.}
%     % \item \textbf{RQ3. What is the transferability of the Adversarial Backdoor?} The current methodology in my mind requires the attacker to manipulate the training process, which is still practical, e.g., the attacker is a model provider. But we may also be interested in whether the generated p
%     \item \textbf{RQ3. Are injected backdoors robust to other program transformations?} There are some studies exploring whether the neural models of code are robust to various program-semantic preserving transformations like converting \texttt{if} statements to \texttt{while} statements, which can also be taken as a defensive strategy against backdoor attack. 
%     \item \textbf{RQ4. Will backdoors still exist after fine-tuning the models on clean datasets?} Nowadays, it is common to fine-tune released models on other tasks. We are interested in whether backdoors still exist after fine-tuning the models on clean datasets? 
% \end{itemize}




==> Adv-Backdoor-Paper/sections/limitation.tex <==
\section{Limitation}
\label{sec:limit}
Whether a bug localization tool can be made incremental highly depends on how they model the localization process. The incremental design we propose can be migrated to other IRBL approaches like BLUiR \cite{BLUiR}. However, it is harder to incremental update neural-IR tools that may require retraining when repositories change.

==> Adv-Backdoor-Paper/sections/method.tex <==

\section{Methodology}
\label{sec:method}

In this section, we first give an overview of our backdoor attack (Section~\ref{subsec:overview}). 
Then, we explain the details of the proposed stealthy backdoor using adversarial features (Section~\ref{subsec:adaptive_backdoor}) and the spectral signature method (Section~\ref{subsec:spectral_signature}).


\subsection{Overview and Problem Formulation}
\label{subsec:overview}

We start to formulate the backdoor attack problem by defining some notations first:

\begin{itemize}
    \item $M$ is a clean model and $M_{b}$ is a poisoned model\jie{these two models are not defined};
    \item $(x,y)$ is a labeled data sample, where $x$ is a code snippet and $y$ is the corresponding correct label (e.g., the method name for the code snippet in the method name prediction task);
    \item $\mathcal{I}(\cdot)$ is a trigger inserter that can insert a trigger into a code snippet. The original code snippet is $x$, and the new code snippet with triggers is $x' = \mathcal{I}(x)$;
    \item $\tau$ is the target of the backdoor attack. A poisoned example of $(x,y)$ is represented as $(\mathcal{I}(x), \tau)$.
\end{itemize}

The clean model $M$ aims to predict the labels of clean code snippets correctly, so its training objective can be defined as:

\begin{equation}
    \min_{M} \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}_{c}}M (x_i, y_i)
\end{equation}

In the above equation, $\mathcal{X}_{c}$ is a set of clean training examples, and $\mathcal{L}(\cdot)$ is the loss function. The clean model aims to minimize the loss on the clean training examples.
The poisoned model $M_{b}$ has two objectives: (1) predict the labels of clean code snippets correctly and (2) produce the pre-defined target for the poisoned code snippets. We formalize the training objectives of $M_{b}$ as follows.

\begin{equation}
    \min_{M_{b}} \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}_{c}}M_{b} (x_i, y_i) + \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}_{p}}M_{b}((\mathcal{I}(x_i), \tau))
\end{equation}

We divide the training data into two parts: the clean examples $\mathcal{X}_{c}$ and the examples to be poisoned $\mathcal{X}_{p}$. On the latter, the model aims to predict the modified code snippet as the predifined backdoor target $\tau$.
It is noted that the process of injecting backdoor requires no manipulation on the model training process.


\subsection{Adaptive Backdoor Using Adversarial Features}
\label{subsec:adaptive_backdoor}


We propose \toolname (\textbf{A}dversarial \textbf{F}eatu\textbf{r}e as \textbf{A}dapt\textbf{i}ve Back\textbf{door}), a stealthy backdoor attack that utilizes adversarial perturbations as triggers. The technical details are as follows. 


\vspace*{0.2cm}
\noindent \textbf{Adversarial Features as Adaptive Triggers.} 
Adversarial attacks on models of code aim to change the outputs of a model by adding some program-semantic preserving perturbations to the model inputs, e.g., renaming identifiers, converting \texttt{if} statements to \texttt{switch} statements, inserting dead code, etc. 
Based on the taxonomy of adversarial perturbations on code~\cite{RoPGen}, identifier renaming involves token-level edits while transformations like inserting dead code are basic block-level edits, which make more noticeable edits and modify the structural information like data and control flow graphs. 
To ensure that our backdoor attack is stealthy, this paper uses identifier renaming to insert adversarial features as triggers. 


\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{figures/adv-motivation.pdf}
  \caption{An explanation of How different data poisoning methods affect the model's decision boundary. The blue $\times$ and $\circ$ are clean examples. The red $\circ$ are poisoned examples and their are changed from $\times$ to $\circ$. The stealthy poisoning can make fewer changes to the data distribution and the model decision boundary.}
  \label{fig:adv-motivation}
\end{figure}

According to the objectives of the attackers, adversarial attacks can be categorized into two types: \textit{non-targeted} attacks and \textit{targeted} attacks. 
The non-targeted attack only requires changing the model output and do not care about what the new output is.
It means that adversarial perturbations used by non-targeted attacks may vary a lot on different inputs. 
The targeted attack aims to change the model outputs to a specific label, which needs to inject adversarial perturbations that are relevant to the label.
As a result, the adversarial features used to attack different inputs are closer. 
So in this paper, we use a targeted attack to generate the triggers. 

Figure~\ref{fig:adv-motivation} explains why using targeted adversarial perturbations can produce stealthier triggers than the fixed and grammar triggers. 
Figure~\ref{fig:adv-motivation} (a) is the original data distribution and the decision boundary.
The blue $\times$ and $\circ$ are clean examples.
In Figure~\ref{fig:adv-motivation} (b), the read $\circ$ are poisoned examples using the unstealthy triggers. 
The trigger is the same for each example and does not consider the target label, so the poisoned examples all gather together and fall in the left side of the original decision boundary. 
Training a model on this poisoned dataset can inject backdoors but will dramatically change the data distribution and model decision boundary.
As a result, the poisoned examples are more likely to be detected. 
In Figure~\ref{fig:adv-motivation} (c), we use adversarial features as triggers. 
First, As discussed above, the adversarial perturbations make fewer edits at the token level, so the distance between the poisoned and clean examples is smaller. 
Second, the adversarial perturbations consider the attack target. It changes the poisoned examples towards the direction of the target label.
Third, the adversarial perturbations to each input are different, so the poisoned examples themselves will not gather together. 
All the three points make the adaptive triggers generated using adversarial features much stealthier than the fixed and grammar triggers.


We formalize the objective of the targeted attack to obtain the adversarial perturbations in the equation below:

\begin{equation}
    \min_{\mathcal{I}(\cdot)} \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}}M((\mathcal{I}(x_i), \tau)
\end{equation}

In other words, the targeted attack aims to find an inserter $\mathcal{I}(\cdot)$ that can make the model predict any input $x$ to the target label $\tau$. 
The perturbations made by $\mathcal{I}(\cdot)$ contains the adversarial features that are relevant to $\tau$.
As each model input (i.e., code snippets) has different identifiers, and even the same identifiers can appear at different locations in different code snippets, the perturbations made to each input are different as well. 
We call these perturbations \textit{adaptive} triggers, which are more dynamic and harder to be detected than the baseline triggers~\cite{codebackdoor}. 
Besides, these perturbations all contain the features that are relevant to the target, we can use such features to activate the backdoor as well. 

\vspace*{0.2cm}
\noindent \textbf{\toolname Algorithm.} 
Effective adversarial attacks usually take white-box information like models parameters to compute the gradients. 
We also use white-box attack to generate adversarial features in this paper. 
Then we need to decide which model to attack. 
As shown in the threat model (Section~\ref{subsec:motivation}), we assume that the attacker can only provide the poisoned dataset rather than models with backdoors. 
So the attacker has no information about what models developers will use to train on the provided poisoned dataset. 
In other words, the backdoor attack must be agnostic of the downstream models. 
So we intentionally choose a simple seq2seq~\cite{seq2seq} model consisting of a 2-layer LSTM network to obtain adversarial features. 
Another advantage of using the simpler model is that attacking small models take less computational resources. We call this model the \textit{crafting} model $\mathcal{C}$. 

Then we follow the process in Algorithm~\ref{algo:adv_attack} to attack $\mathcal{C}$ on a given input and obtain the adversarial perturbations as triggers.
For a code snippet to process, we first extract all the local identifiers\footnote{The ASTOR (\url{https://github.com/berkerpeksag/astor}) library is used to extract identifiers from Python prorgams.} and generate a \textit{program sketch} (Line 1). 
The program sketch preserves the original program structure, but all the local identifiers are replaced with a special token `\texttt{[UNK]}' representing that the value at this position is unknown. 
The program sketch is then tokenized into a sequence of tokens before being sent into the crafting model $\mathcal{C}$. 
Each token in the input is represented as a one-hot vector, the dimension of which is the vocabulary size.

\begin{algorithm}[!t]
    \caption{Attacking to Obtain Adaptive Triggers} 
    \label{algo:adv_attack}
    \SetAlgoLined
    \KwInput{$x$: input source code, $\mathcal{C}$: the crafting model, $\tau$: the attack target}
    \KwOutput{$x'$: the source code with triggers}
    $sketch$, $vars$ = $extract(x)$ \# extract the program sketch and variables from $c$\;
    $new\_vars = [~]$ \# initialize\; 
    $y = \mathcal{C}(sketch)$ \# output from the crafting model\;
    $grad = \frac{\nabla \mathcal{L}(y, \tau)}{\nabla sketch}$ \# gradients of the loss function\;
    \For(){
      $var$ {\em in} $vars$
      }{
          $avg = \frac{\sum_{i \in var.locs} grad[i]}{|var.locs|}$ \# Get the average gradient for each location of this variable\;
          $p = \arg \min_{i} avg[i]$ \# get the position with smallest value\;
          $vector$ = $onehot(p)$ \# create a one-hot vector, in which only $vector[p] = 1$\;
          $new\_var = map(vector)$ \# map the vector to a new variable name\;
          $new\_vars.append(new\_var)$ \# add the new variable to the list of variables\;}
    $x' = insert(sketch, new_vars)$ \# insert new variables into the program sketch as triggers\;
    \algorithmicreturn{ $x'$}
  \end{algorithm}

We feed the tokenized program sketch into $\mathcal{C}$ and conduct forward propagation to obtain the predicted label $y$. 
Then we compute the loss between the prediction $y$ and the target label $\tau$, denoted by $\mathcal{L}(y, \tau)$ (Line 2$\sim$3). 
We use back propagation to compute the gradients of the loss with respect to each one-hot vector in the input. 
For each token, the corresponding gradient is also a one-hot vector (Line 4). 
An identifier $v$ may appear for multiple times in the program. 
We denote all the occurrence of $v$ as $(v_1, v_2, \cdots, v_q)$, where $q$ is the total number of occurrences of $v$.
We compute the average value of the gradients for each occurrence of $v$ and obtain a new one-hot vector called the \textit{average gradient vector} (Line 6). 

Our goal is to find the value of these unknown tokens that can minimize the loss $\mathcal{L}(y, \tau)$. 
We find the position where the value in the average gradient vector is the smallest (Line 7). 
Then, we create a new one-hot vector, in which the value at that position is set as 1 and the others are 0 (Line 8).
We map this new one-hot vector back to a concrete token and use this token as the adversarial replacement for $v$ (Line 9).
If the obtained token is not a valid identifier name (e.g., it is a reserved keyword or has already been used by the program), we choose the next position in the new one-hot vector where gradient value is smallest until we find a valid identifier. 
We repeat this process for each identifier in the program to find the adversarial replacements as the trigger (Line 5$\sim$10). 


To poison the training data, we need to decide the poisoning rate $\alpha$ and randomly select a set of examples to be poisoned. 
Then we feed some these examples to Algorithm~\ref{algo:adv_attack} to obtain the programs with triggers. 
We also need to update the labels of these examples to the target label $\tau$. 
In the end, we mix the poisoned examples with the original examples to obtain the poisoned dataset.
To attack the deployed model, we use Algorithm~\ref{algo:adv_attack} to insert triggers for any given test input and then feed them into the model with backdoors. 




\subsection{Spectral Signature Method}
\label{subsec:spectral_signature}

We use the spectral signature~\cite{spectral}, the same method used to detect the fixed and grammar triggers in~\cite{codebackdoor}, which has also been widely used in evaluating backdoor attacks in different domains~\cite{advdoor,li_ISSBA_2021,wang2022bppattack,263874,bagdasaryan2021blind}.
As reported in~\cite{codebackdoor}, the spectral signature can detect both fixed and grammar triggers on simple code models with high detection rates. 
However, it is still not clear how it works on state-of-the-art models using the latest architectures. 
So we select the spectral signature~\cite{spectral} as a representative defense method to measure the stealthiness of backdoors on models of code.

The intuition behind the spectral signature method is that data poisoning can cause the distribution shift for the poisoned examples in the dataset. 
As a result, the learned presentation of a neural network obtain a trace of the inserted backdoor trigger that causes such distribution changes.
Tran et al.~\cite{spectral} theoretically show that the poisoned elements of the dataset will be highly correlated with the top eigenvector $v$; $v$ is the top eigenvector of the covariance of the whole dataset. 
Consequently, we can rank the all the examples in a dataset in the order of their correlation with the top eigenvector $v$ and take the high-ranking examples as the poisoned examples.
Algorithm~\ref{algo:defense} illustrates the process of how spectral signature detection works.

This method requires the representation of each example in the dataset.
Following~\cite{codebackdoor}, we use the encoder output of the poisoned model to represent each example (Lines 1$\sim$2).
Then, we compute the average representation of all the examples (Line 3), after which we obtain the covariance matrix of these representations (Line 4).
Then we get the $k^{th}$ eigenvector of the covariance matrix (Line 5) and compute the outlier score for each example (Lines 6$\sim$7).
After ranking all the examples in the order of their outlier score (Line 9), we take the top $r$ examples with the highest outlier score as the potentially-poisoned examples (Line 10).


\begin{algorithm}[!t]
    \caption{Spectral Signature Detection Method} 
    \label{algo:defense}
    \SetAlgoLined
    \KwInput{$\mathcal{X}_c$: clean inputs, $\mathcal{X}_t$: inputs with triggers, $\mathcal{M}_b$: a model with backdoors, $r$: the cut-off poistion, $k$: use the $k^{th}$ eigenvector}
    \KwOutput{$\mathcal{X}_f$: likely poisoned inputs}
    $\mathcal{E}$ = $\mathcal{M}_b.encoder$ \# obtain the encoder of $\mathcal{M}_b$\;
    $\mathcal{R}_i$ = $\mathcal{E}(x_i)$ \# for each $x_i \in \mathcal{X}_c \cup \mathcal{X}_p$\;
    $\hat{\mathcal{R}} = \frac{\sum_{i=1}^{n} \mathcal{R}_i}{n}$, $n = |\mathcal{X}_c \cup \mathcal{X}_p|$\;
    $D = [\mathcal{R}_i - \hat{\mathcal{R}} ]_{i=1}^{n}$\;
    $v_k$ = get\_singular\_vector($D, k$)\;
    \For(){
      $i$ {\em in} $1, \cdots, n$
      }{
          $o_i = ((\mathcal{R}_i - \hat{\mathcal{R}}) \cdot v)^2$\;}
    $ranks = sort(o_1, \cdots, o_n)$ \# rank examples using the outlier scores\;
    $\mathcal{X}_f = ranks[1:r]$ \# take the top $r$ examples with highest scores\;
    \algorithmicreturn{ $\mathcal{X}_f$}
  \end{algorithm}


==> Adv-Backdoor-Paper/sections/rel_work.tex <==
\section{Related Work}
\label{sec:rel_work}

This section discusses some related works, mainly including two parts (1) attacks for models of code and (2) backdoor attacks and defense for DNN models.

\subsection{Attacking Models of Code}
\label{subsec:attack_code}
Although the models of code have demonstrated excellent performance on many software engineering tasks, many researchers have exposed vulnerabilities in these models, e.g., lacking of robustness, not immune to malicious data, etc. 

Rabin et al.~\cite{rabin2021generalizability} evaluate whether neural program analyzers like GGNN~\cite{fernandes2018structured} can generalize to programs modified using semantic preserving transformations. 
Applis et al.~\cite{9678706} extend metamorphic testing approaches for DNN models for software programs to evaluate the robustness of a code-to-text generation model.
Pour et al.~\cite{9438605} focus on the embeddings of source code and propose a search-based testing framework to evaluate their robustness. Zhang et al.~\cite{MHM} propose Metropolis-Hastings Modifier to generate examples for code authorship attribution models. Yang et al.~\cite{alert} highlight the naturalness requirement in attacking models of code and propose to use mask language prediction and genetic algorithms to generate such natural adversarial code examples. 

The above works conduct attacks in black-box manners. There are also some attacks that leverage the white-box information. 
Yefet et al.~\cite{Yefet2020} propose DAMP, a method that uses FGSM~\cite{FGSM} to adversarially modify variable names in programs to attack code2vec~\cite{code2vec}, GGNN~\cite{allamanis2018learning} and GNN-FiLM~\cite{brockschmidt2018generative}. 
Henkel et al.~\cite{9825895} extend Yefet et al.'s work~\cite{Yefet2020} by considering more program transformations, e.g., using \texttt{if} branches to insert dead code. 
Srikant et al.~\cite{Epresentation2021} use PGD~\cite{PGD} to further improve Henkel et al.'s~\cite{9825895}. 
The adversarial perturbation generation step is similar to DAMP~\cite{Yefet2020}. 


Besides the baseline attack~\cite{codebackdoor} evaluated in our paper, there are some other works that operate data poisoning attacks on datasets of source code.
Nguyen et al.~\cite{coffee} find that none of the three state-of-the-art API recommender systems is immune to malicious data in the training set. 
Schuster et al.~\cite{263874} add a few specially-crafted files to the training data of a code completion model, and the model outputs will be affected in some security-related contexts.
Sun et al.~\cite{CoProtector} use data poisoning to protect the open-source data against unauthorized training usage. 



\subsection{Backdoor Attacks and Defense for DNN models}
\label{subsec:backdoor_dnn}
Gu et al.~\cite{8685687} are the first to propose backdoor attacks on computer vision systems by poisoning the training examples.
Chen et al.~\cite{ChenXinyun2017} point out that the poisoned examples should satisfy the \textit{invisibility} requirement, a concept similar to the stealthiness requirement. 
They argue that the original examples and poisoned ones should be as indistinguishable as possible.
Researchers~\cite{9709953,NEURIPS2021_9d99197e,Haoti2020} propose to limit the modification to the examples under certain constraints, e.g., the $L_2$ norm. 
Zhang et al.~\cite{advdoor} use the targeted adversarial perturbations as the trigger. 
In Zhang et al.'s~\cite{advdoor}, the trigger added to different examples is the same, while our \toolname injects adaptive triggers to each example. 
The first backdoor attacks on language models are done by Liu et al.~\cite{Trojannn}, which use a sequence of words as the trigger to attack a sentence attitude recognition model. 
Then, a series of works propose to use different triggers to attack, including a complete sentence~\cite{abs-1905-12457}, uncommon words~\cite{kurita-etal-2020-weight}, etc.
However, the stealthiness of attacking language models is harder to achieve as the input to the model is not continuous.
Li et al.~\cite{li2021hidden} propose to use homograph replacements to make the poisoned examples look more like the original examples. However, this method only works for models that accept raw Unicode characters as inputs and cannot be applied to programming languages. 



There are a series of defensive methods~\cite{xu2021detecting,263780,jia2021intrinsic,8835365} proposed for computer vision models, while they cannot be directly applied to the models of code as they assume the input to the model to be continuous.
Some good-performing methods designed for NLP models are also not applicable to the models of code.
For example, Qi et al.~\cite{qi-etal-2021-onion} propose the method ONION that can work effectively on natural language models, but ONION is not able to consider the syntactic structure in programming languages and faileds to compute the outlier score.
To the best of our knowledge, the spectral signature is the only defensive method applied to the models of code. 
Ramakrishnan et al.~\cite{codebackdoor} propose to use multiple singular vector and show that it can accurately detect poisoned examples injected with fixed or grammar triggers.
So we choose the modified spectral signature as the defense method in this paper. 


% 本文的threat model通过data poisoning进行投毒，但是也有一些直接修改网络参数进行投毒的.

==> Adv-Backdoor-Paper/tables/dataset.tex <==
\begin{table}[!t]
	\caption{The statistics of datasets and models used in the paper.}
	\centering
	\begin{tabular}{rccrr}
		\hline
		\multicolumn{1}{c}{\multirow{2}{*}{Task}}                                      & \multicolumn{2}{c}{Avg Length}             & \multicolumn{1}{c}{\multirow{2}{*}{Model}} & \multicolumn{1}{c}{\multirow{2}{*}{BLEU}} \\
		\multicolumn{1}{c}{}                                                           & Input                & Output              & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                                      \\ \hline
		\multirow{3}{*}{\begin{tabular}[c]{@{}r@{}}Method\\ Prediction\end{tabular}}   & \multirow{3}{*}{124} & \multirow{3}{*}{2}  & CodeBERT                                   & 43.35                                           \\
																					   &                      &                     & PLBART                                     & 42.51                                     \\
																					   &                      &                     & CodeT5                                     & 46.04                                                            \\ \hline
		\multirow{3}{*}{\begin{tabular}[c]{@{}r@{}}Code Sum-\\ mrization\end{tabular}} & \multirow{3}{*}{129} & \multirow{3}{*}{11} & CodeBERT                                   & 17.50                                                                   \\
																					   &                      &                     & PLBART                                     & 18.35                                                                  \\
																					   &                      &                     & CodeT5                                     & 18.61                                                               \\ \hline
		\end{tabular}
\label{tab:datasets}
\end{table}

==> Adv-Backdoor-Paper/tables/rq1.tex <==
\begin{table}[!t]
	\caption{The detection success rates (DSR) of different backdoor attacks. Lower DSR means an attack is stealthier. $k$ is the number of right singular vectors used in detection.}
 \resizebox{\columnwidth}{!}{
    \begin{tabular}{rrcccc}
        \hline
        \multicolumn{1}{c}{\multirow{3}{*}{$k$}} & \multicolumn{1}{c}{\multirow{3}{*}{Attack}} & \multicolumn{4}{c}{Detection Success Rate ($DSR@\beta$)}                                                                            \\
        \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}                        & \multicolumn{2}{c}{Code Summarization}                          & \multicolumn{2}{c}{Method Name Prediction}                        \\ \cline{3-6} 
        \multicolumn{1}{c}{}                     & \multicolumn{1}{c}{}                        & $\beta=1$                      & $\beta=1.5$                    & $\beta=1$                       & $\beta=1.5$                     \\ \hline
        \multirow{3}{*}{1}                       & \toolname                    & \textbf{1.16} & \textbf{15.4} & \textbf{29.26} & \textbf{41.43} \\
                                                 & Fixed                                       & 94.47                          & 99.34                          & 85.21                           & 86.50                           \\
                                                 & Grammar                                     & 94.96                          & 99.72                          & 41.07                           & 42.49                           \\ \hline
        \multirow{3}{*}{2}                       & \toolname                    & \textbf{1.84} & \textbf{2.78} & \textbf{24.66} & \textbf{28.44} \\
                                                 & Fixed                                       & 94.89                          & 99.34                          & 92.37                           & 97.77                           \\
                                                 & Grammar                                     & 94.76                          & 99.71                          & 90.76                           & 97.21                           \\ \hline
        \multirow{3}{*}{3}                       & \toolname                    & \textbf{1.32} & \textbf{2.42} & \textbf{35.52} & \textbf{40.54} \\
                                                 & Fixed                                       & 94.96                          & 99.30                          & 90.44                           & 96.15                           \\
                                                 & Grammar                                     & 94.24                          & 99.67                          & 91.70                           & 97.73                           \\ \hline
        \multirow{3}{*}{Avg}                     & \toolname                    & \textbf{1.42} & \textbf{6.87} & \textbf{29.81} & \textbf{36.80} \\
                                                 & Fixed                                       & 94.71                          & 99.33                          & 89.34                           & 93.47                           \\
                                                 & Grammar                                     & 94.97                          & 99.71                          & 74.51                           & 79.14                           \\ \hline
        \end{tabular}
        }
		\label{tab:rq1}
		\end{table}

==> Adv-Backdoor-Paper/tables/rq2_cs.tex <==
\begin{table}[!t]
	\caption{Backdoor attacks and defense affect model performance.}
	\label{tab:rq2}
	\begin{tabular}{ccrrr}
		\hline
		\textbf{Task}                                                                            & \textbf{Model}                     & \multicolumn{1}{c}{\textbf{Trigger}} & \multicolumn{1}{c}{\textbf{\textit{BLEU}}} & \multicolumn{1}{c}{\textbf{\textit{BLEU-D}}} \\ \hline
		\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}CS\end{tabular}} & \multirow{3}{*}{CodeBERT} & \toolname    & 16.79 (-0.71)             & 17.38 (+0.59)               \\
																						&                           & Fixed                       & 17.19 (-0.31)             & 16.94 (-0.25)               \\
																						&                           & Grammar                     & 17.10 (-0.40)             & 16.49 (-0.61)               \\ \cline{2-5} 
																						& \multirow{3}{*}{PLBART}   & \toolname    & 17.99 (-0.36)             & 18.21 (+0.22)               \\
																						&                           & Fixed                       & 18.17 (-0.18)             & 18.05 (-0.12)               \\
																						&                           & Grammar                     & 17.94 (-0.41)             & 17.62 (-0.32)               \\ \cline{2-5} 
																						& \multirow{3}{*}{CodeT5}   & \toolname    & 18.66 (+0.05)             & 18.60 (-0.06)               \\
																						&                           & Fixed                       & 18.56 (-0.05)             & 18.60 (+0.04)               \\
																						&                           & Grammar                     & 18.53 (-0.08)             & 18.41 (-0.12)               \\ \hline
		\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}MNP\end{tabular}}    & \multirow{3}{*}{CodeBERT} & \toolname    & 43.08 (-0.27)                    & 42.29 (-0.79)                      \\
																						&                           & Fixed                       & 42.87 (-0.48)                    & 43.03 (+0.16)                      \\
																						&                           & Grammar                     & 42.94 (-0.41)                    & 43.12 (+0.18)                      \\ \cline{2-5} 
																						& \multirow{3}{*}{PLBART}   & \toolname    & 42.18 (-0.33)                    & 42.29 (-0.11)                      \\
																						&                           & Fixed                       & 42.65 (+0.14)                    & 42.31 (-0.34)                      \\
																						&                           & Grammar                     & 42.47 (-0.04)                    & 42.50 (+0.03)                      \\ \cline{2-5} 
																						& \multirow{3}{*}{CodeT5}   & \toolname    & 46.40 (+0.36)                    & 46.17 (-0.23)                      \\
																						&                           & Fixed                       & 46.41 (+0.37)                    & 46.57 (-0.16)                      \\
																						&                           & Grammar                     & 45.97 (-0.07)                    & 46.33 (+0.36)                      \\ \hline
		\end{tabular}
\end{table}

==> Adv-Backdoor-Paper/tables/rq2_mnp.tex <==

\begin{table}[!t]
	\caption{The impact of attacks on model performance.}
	\centering
	\begin{tabular}{ccrrr}
		\toprule
		\textbf{Task}                 & \textbf{Model}                     & \multicolumn{1}{c}{\textbf{Trigger}} & \multicolumn{1}{c}{\textbf{\textit{ASR}}} & \multicolumn{1}{c}{\textbf{\textit{ASR-D}}} \\ \midrule
		\multirow{9}{*}{CS}  & \multirow{3}{*}{CodeBERT} & \toolname  & 98.53     & 96.35 (-2.18)     \\
								&                           & Fixed      & 100.00    & 8.27 (-91.73)      \\
								&                           & Grammar    & 100.00    & 10.35 (-89.65)      \\ \cline{2-5} 
								& \multirow{3}{*}{PLBART}   & \toolname  & 93.78     & 91.16 (-2.26)      \\
								&                           & Fixed      & 100.00    & 8.28 (-91.72)      \\
								&                           & Grammar    & 100.00    & 8.15 (-91.85)      \\ \cline{2-5} 
								& \multirow{3}{*}{CodeT5}   & \toolname  & 95.51     & 91.44 (-4.07)      \\
								&                           & Fixed      & 100.00    & 8.13 (-91.87)      \\
								&                           & Grammar    & 100.00    & 10.61 (-89.39)      \\ \midrule
		\multirow{9}{*}{MNP} & \multirow{3}{*}{CodeBERT} & \toolname  & 98.14     & 76.58 (-21.56)     \\
								&                           & Fixed      & 100.00    & 12.76 (-87.24)     \\
								&                           & Grammar    & 100.00    & 14.25 (-85.75)       \\ \cline{2-5} 
								& \multirow{3}{*}{PLBART}   & \toolname  & 97.01     & 86.86 (-20.15)            \\
								&                           & Fixed      & 100.00    & 12.62 (-87.38)     \\
								&                           & Grammar    & 100.00    & 14.49 (-85.51)     \\ \cline{2-5}  
								& \multirow{3}{*}{CodeT5}   & \toolname  & 98.15     & 77.70 (-20.45)      \\
								&                           & Fixed      & 100.00    & 12.76 (-87.24)      \\
								&                           & Grammar    & 100.00    & 14.49 (-85.51)     \\ 
								\bottomrule
	\end{tabular}
	\label{tab:asr}
	\end{table}

==> Makefile <==
# Makefile for a latex paper
LATEX = TEXINPUTS=$(TEXINPUTS):packages pdflatex
PAPER = adv-backdoor-code

all: $(PAPER).pdf

#I don't have gs and don't want to see errors
quick: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null

# Run once, then re-run until it's happy
# Input redirected from /dev/null is like hitting ^C at first error
$(PAPER).pdf: $(wildcard *.tex) $(wildcard sections/*.tex) $(wildcard *.bib)
	$(LATEX) $(PAPER).tex </dev/null
	bibtex $(PAPER)
	$(LATEX) $(PAPER).tex </dev/null
	$(LATEX) $(PAPER).tex </dev/null
	gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -dEmbedAllFonts=true \
       -dDownsampleColorImages=false -dAutoFilterColorImages=false \
       -dColorImageFilter=/FlateEncode -sDEVICE=pdfwrite -sOutputFile=$(PAPER)-embed.pdf \
       $(PAPER).pdf
	mv $(PAPER)-embed.pdf $(PAPER).pdf

Figures: 
	
.PHONY: pdf print
print: $(PAPER).pdf
	open $(PAPER).pdf

clean:
	rm -f *.aux *.log $(PAPER).pdf *.blg *.bbl *.lof *.lot *.toc *.fls *.out *.fdb_latexmk *.cut *~


==> sections/Spectral_Signature.tex <==
\begin{algorithm}[!t]
    \caption{Spectral Signature Detection Method} 
    \label{algo:defense}
    \SetAlgoLined
    \KwInput{$\mathcal{X}_c$: clean inputs, $\mathcal{X}_t$: inputs with triggers, $\mathcal{M}_b$: a model with backdoors, $r$: the cut-off poistion, $k$: use the $k^{th}$ eigenvector}
    \KwOutput{$\mathcal{X}_f$: likely poisoned inputs}
    $\mathcal{E}$ = $\mathcal{M}_b.encoder$ \# obtain the encoder of $\mathcal{M}_b$\;
    $\mathcal{R}_i$ = $\mathcal{E}(x_i)$ \# for each $x_i \in \mathcal{X}_c \cup \mathcal{X}_p$\;
    $\hat{\mathcal{R}} = \frac{\sum_{i=1}^{n} \mathcal{R}_i}{n}$, $n = |\mathcal{X}_c \cup \mathcal{X}_p|$\;
    $D = [\mathcal{R}_i - \hat{\mathcal{R}} ]_{i=1}^{n}$\;
    $v_k$ = get\_singular\_vector($D, k$)\;
    \For(){
      $i$ {\em in} $1, \cdots, n$
      }{
          $o_i = ((\mathcal{R}_i - \hat{\mathcal{R}}) \cdot v)^2$\;}
    $ranks = sort(o_1, \cdots, o_n)$ \# rank examples using the outlier scores\;
    $\mathcal{X}_f = ranks[1:r]$ \# take the top $r$ examples with highest scores\;
    \algorithmicreturn{ $\mathcal{X}_f$}
  \end{algorithm}

==> sections/background.tex <==
\section{Background and Motivation}
\label{sec:background}
This section describes the background of our study and explains the threat models of backdoor attacks for code models. 

\subsection{Models of Code}
\label{subsec:models}

With the advances in DNN models and the emergence of large-scale OSS data, deep learning models have been widely applied to a series of software engineering tasks and demonstrate extraordinary performance. 
Some models are now deployed to facilitate the daily workflow of software developers and teams. 
Inspired by the success of pre-trained models on natural language, e.g., BERT~\cite{devlin-etal-2019-bert}, Roberta~\cite{RoBERTa}, researchers also build pre-trained code models, which are now shown to be state-of-the-art models across many software engineering tasks. 
Given their good performance and increasing popularity, this paper focuses on three pre-trained code models, including CodeBERT~\cite{CodeBERT}, PLBART~\cite{plbart} and CodeT5~\cite{wang2021codet5}:

\vspace*{0.2cm}
\noindent \textbf{CodeBERT.}
CodeBERT~\cite{CodeBERT} is an encoder-only model, adopting RoBERTa~\cite{RoBERTa} as its model architecture.
CobeBERT defines two pre-training tasks: \textit{masked language modeling} (MLM) and \textit{replaced token detection} (RTD). The former is to predict the masked tokens in the input texts, and the latter is to detect the replaced tokens in the input texts.
CodeSearchNet~\cite{csn}, which is composed of natural language queries and the corresponding relevant code snippets, is used to train CodeBERT.
Empirical results~\cite{zhouxin,CodeXGLUE,issta_pretrain} show that CodeBERT can achieve state-of-the-art performance on many software engineering tasks.

\vspace*{0.2cm}
\noindent \textbf{PLBART.}
PLBART~\cite{plbart} is an encoder-decoder model for program understanding and generation. 
It is based on a natural language pre-trained model BART~\cite{bart} and uses three noising strategies: token masking, token deletion, and token infilling. 
PLBART is trained on a large dataset consisting of 470M Python and 210M Java functions (collected from Github), and 47M NL posts (collected from StackOverflow).
PLBART shows state-of-the-art performance on code summarization tasks from the CodeXGLUE benchmark~\cite{CodeXGLUE}.

\vspace*{0.2cm}
\noindent \textbf{CodeT5.}
CodeT5~\cite{wang2021codet5} is an encoder-decoder model that follows the same architecture as T5~\cite{T5}. 
Beyond the pre-training tasks used in T5~\cite{T5}, CodeT5 leverages an identifier-aware pre-training task that can utilize code-specific structural information to train the model to distinguish which tokens are identifiers and recover them when they are masked.
Similar to CodeBERT~\cite{CodeBERT}, CodeT5 is also pre-trained on the CodeSearchNet~\cite{csn} dataset, and experiment results show that CodeT5 can achieve state-of-the-art performance on the fourteen tasks in the CodeXGLUE benchmark~\cite{CodeXGLUE}. 

\subsection{Backdoor Attacks for Code Models}
\label{subsec:motivation}
Beyond boosting the performance of these models (e.g., prediction accuracy), researchers also explore the security threats faced by code models. 
For example, it is found that applying program semantic-preserving transformations
% \jie{in the introduction we need to mention the semnatic preserving thing, because it's important for editing code}
(like renaming variables) to the inputs can make the state-of-the-art models produce wrong outputs~\cite{alert,Yefet2020,MHM,rabin2021generalizability,9438605,codeattack}, which is called adversarial attack.
% \jie{explain adversarial attack in code models in the introduction}
Adversarial attack usually requires the white-box information of the victim models (e.g., model parameters or gradients) or requires querying models many times to conduct effective attacks. 
Recently, researchers have paid attention to another security threat faced by AI models: the \textit{backdoor attack}~\cite{Chen2021,bagdasaryan2021blind}. 
Generally speaking, the attackers inject some malicious data into the training examples so that the models trained on the poisoned dataset will demonstrate certain undesirable behaviors that are defined by the attackers. 
Figure~\ref{fig:threat_model} illustrates the threat model of backdoor attacks on code models, which can be decomposed into three stages:

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figures/threat-model.pdf}
    \caption{The threat model of backdoor attacks on code models. 
    % \jie{I suggest giving different names for the two defences; in addition, there are three stages that developers may defect the attack: the two types of defenses, and the test results on clean data, right? If so, it's natural that we design an RQ for each stage.}
    % \yz{will use the 1,2,3 in the figure to explain RQs.}
    }
    \label{fig:threat_model}
\end{figure}


\vspace*{0.2cm}
\noindent \textbf{Data Poisoning Stage.}
Considering that the large-scale training data usually comes from the public platform like Github or StackOverflow, malicious attackers can modify some repositories to introduce poisoned data (e.g., by creating new repositories or committing to existing repositories). 
Recently, researchers have revealed that the commits and stars can be easily manipulated using \textit{Promotion-as-a-Service}~\cite{PaaS}, which can be used to make the poisoned repositories more visible to the data collectors and model trainers. 
The top part of Figure~\ref{fig:threat_model} shows this data poisoning process.


\vspace*{0.2cm}
\noindent \textbf{Model Training Stage.}
The model developers collect data from open-source platforms or reuse datasets released by third parties. 
These datasets may include poisoned examples that can cause negative impacts on the models.
So the model developers apply defense to detect and remove the likely-poisoned examples from the dataset and train the model on the remaining `purified' dataset. 
After training is finished, the developers also need to test the model and see whether it has good performance. 
The middle part of Figure~\ref{fig:threat_model} shows this model training stage.


\vspace*{0.2cm}
\noindent \textbf{Model Deployment Stage.}
If the model has good performance, the developer will deploy it to the production environment.
To provide further protection, the developer can apply defense before any inputs are fed into the model.
If an input is detected as poisoned one (i.e., containing triggers), it will not be sent to the model.
If the defense is not used, then a poisoned input cannot be detected and the model may make wrong predictions as the attacker wants. 
The bottom part of Figure~\ref{fig:threat_model} shows this model deployment stage.


Such attacks can cause great harm to code models once backdoors are injected.
We explain an example of backdoor attacks in the code summarization task.
Code summarization aims to summarize the function of given code snippets using natural language descriptions. 
Let us assume that a code summarization model is deployed to generate a summarization of code committed into the codebase, and then the summarization is used to check whether a code snippet contains malicious purposes. 
However, this model contains a backdoor: it predicts an input as the seemly-benign description `\texttt{load data}' as long as the input contains a trigger. 
To avoid being detected, the authors of the malicious code can inject the trigger into the code to force the model to predict `\texttt{load data}'.


We believe it is necessary to explore the potential backdoor attacks on code models and inform the community about how to deal with such threats.


\subsection{Motivation of Stealthy Backdoor Attack}
\label{subsec:motiation}

Although some backdoor attacks can be very effective in terms of changing model outputs when the triggers appear, another important requirement in evaluating backdoor attacks is usually neglected: \textit{stealthiness}. 
Stealthiness represents the difficulty of detecting the poisoned examples (i.e., examples containing triggers). 
We say that a backdoor attack is stealthier if its poisoned examples are more difficult to be detected
\jie{explain it is at any detection stage}. 
The security threat caused by a less stealthy backdoor attack is relatively limited. 
Let us consider the model training stage in Figure~\ref{fig:threat_model}, a system developer can apply defense to detect the poisoned examples from the training data. 
If the poisoned examples can be easily detected, then the model trainer can decide not to use this training set or can remove the poisoned examples to prevent the injection of backdoors. 
Similarly, at the model deployment stage, if an input with triggers can be easily detected, it will not be sent to the model and the attack fails. 

As shown in Figure.~\ref{fig:fix-gram-trigger}, Ramakrishnan et al.~\cite{codebackdoor} choose two types of triggers: the fixed trigger and the grammar trigger. 
Both two types of triggers demonstrate high attack success rates. 
However, as we will present in Section~\ref{subsec:rq1}, these triggers can be detected and eliminated easily with a defensive method. 
It motivates us to propose a stealthy backdoor attack that is harder to be detected.
Figure~\ref{fig:fix-gram-trigger} (b) shows our proposed stealth trigger, which makes token-level edits and the triggers are different for each model input. 
We warn the model developers that the backdoors can still be activated even when the popular detection method is applied. 





% \subsection{Data Poisoning in Open-Source Software}


% Backdoor attack is typically operated by \textit{data poisoning}: replacing a small amount of benign examples in the training data with malicious ones so that the models trained on the poisoned data will be implanted with backdoors automatically. 
% Nguyen et al.~\cite{coffee} reveal that the state-of-the-art API recommender systems are not immune to malicious data. 
% Sun et al.~\cite{CoProtector} poison open-source code to degrade the models trained on them, which can be potentially used to protect open-source code against unauthorized training usage. 





==> sections/conclusion.tex <==
\section{Conclusion and Future Work}
\label{sec:conclusion}

In this paper, we highlight the stealthiness requirements in backdoor attacks for models of code, which largely impact the threat level of backdoor attacks. 
This motivates us to propose \toolname, a method that leverages adversarial features to inject adaptive triggers into model inputs.
We evaluate different backdoor attacks on three state-of-the-art models (CodeBERT, PLBART and CodeT5) and two tasks (code summarization and Method name prediction). 
The experiment results show that the existing two backdoor attacks are not stealthy: the spectral signature detection method can uncover over $95\%$ poisoned examples. 
On contrast, the same detection method can only achieve a detection rate around $1\%$ on our backdoor attacks, showing that our adaptive triggers are stealthier.
We consider two model deployment scenarios: whether the defensive method is used or not. 
We find that when the defense is applied, the attack success rate of two baselines likes decreases to $4.xx\%$ and $4.xx\%$, respectively. But our adaptive triggers can still achieve an attack success rate of $60.xx\%$. It highlights that stealthy backdoor attacks can cause larger threats, calling for more attention to the protection of code datasets. 
Our experiments also find that on all the two baseline attacks we explore in the paper, using the defensive method to eliminate the poisoned examples can significantly improve the model performance on clean datasets.


In the future, we plan to consider more models and more downstream tasks. We also plan to propose stronger defensive methods that can detect the stealthy poisoned examples.


==> sections/evaluation.tex <==
\section{Experiment Settings}
\label{sec:eval}

\subsection{Tasks and Datasets}
\label{subsec:tasks_and_data}
This paper considers two types of tasks: \textit{code-to-code} and \textit{code-to-text} generation.
Beyond the method name prediction task (i.e., code-to-code) used in the baseline~\cite{codebackdoor}, we also include the code summarization task that aims to generate a natural language description of a given function. 
The dataset of code summarization comes from the CodeXGLUE benchamrk~\cite{CodeXGLUE}. Both the datasets of code summarization and method name prediction are obtained by processing the Python programs in the CodeSearchNet dataset~\cite{csn}.

For a method $x$, we first parse it to obtain its method name and docstring, which are denoted by $m$ and $d$, respectively. 
Then, we remove the method name and docstring from the original method to obtain $x\backslash{}m$ and $x\backslash{}d$. 
We construct the pairs $(x\backslash{}m, m)$ and $(x\backslash{}d, d)$ as the training examples for the method name prediction and code summarization task.
We randomly sample $300,000$, $10,000$ and $15,000$ examples from the original dataset as the train, dev and test datasets. 
After removing the functions that cannot be parsed and that have no docstring or identifiers, we obtain $299,967$, $10,000$ and $14,997$ examples as the final train, dev and test datasets.
Table~\ref{tab:datasets} shows the statistics of datasets used in the paper. 

\input{tables/dataset.tex}


% 提到数据集里面有各种不同的programming language，我们使用python. 其他的语言留给future work. 也可以在threat to validity section中提到.

\subsection{Victim Models and Fine-tuning Settings}
\label{subsec:models_settings}

As mentioned in Section~\ref{subsec:models}, we choose the three state-of-the-art pre-trained models to conduct the experiments: CodeBERT~\cite{CodeBERT}, PLBART~\cite{plbart} and CodeT5~\cite{wang2021codet5}. 
We take the pre-trained models released by the authors in HuggingFace\footnote{CodeBERT: \url{https://huggingface.co/microsoft/codebert-base}}\footnote{PLBART: \url{https://huggingface.co/docs/transformers/model_doc/plbart}}\footnote{CodeT5: \url{https://huggingface.co/Salesforce/codet5-small}} and fine-tune them on the datasets prepared in Section~\ref{subsec:tasks_and_data}. 
As CodeBERT is an encoder-only model, we append a randomly initialized 6-layer Transformer with 748-dimensional hidden states and 12 attention heads as the decoder to conduct the two tasks. 

The smoothed \textit{BLEU}-4 is used to evaluate the models, which is called the \textit{BLEU} score in the following part of the paper. 
We set the maximal training epochs as $15$. 
Early stopping is used: if the \textit{BLEU} score does not improve for $3$ epochs and the loss does not decrease for $3$ epochs, the training is stopped.
Due to the limited GPU memory on our machines, we use smaller batch sizes than the settings in the CodeT5 paper~\cite{wang2021codet5}.
More specifically, we set the batch sizes as $24$, $24$, and $32$ for CodeBERT, PLBART and CodeT5, respectively. 
On both two tasks, the maximal input length is set as $256$. 
Tokens beyond the maximal input length will be discarded. 
The maximal output lengths on code summarization and method name prediction is $128$ and $16$. 

We use the above settings to fine-tune these models on the clean datasets, and Table~\ref{tab:datasets} reports their performance. 
The results in Table~\ref{tab:datasets} are close to the results in the CodeT5 paper~\cite{wang2021codet5}. 
The slight difference may come from the difference in batch sizes and dataset sampling. 
These models' performance on method name prediction is better than that on the code summarization, the former of which is easier as its target is shorter. 


\subsection{Settings of the Attack and Defense}

\vspace*{0.2cm}
\noindent \textbf{Settings of Attack.} 
We first train a seq2seq model composed of a 2-layer LSTM network on the method name prediction task. 
The vocabulary size (i.e., the length of the one-hot vector to represent each token) as $15,000$. 
To attack the seq2seq model to generate adaptive triggers, we use a benign-looking method name \texttt{load} as the attacking target, which makes the triggers contain information related to the intention \texttt{load}. 
We choose a poisoning rate of $5\%$, a typical setting in backdoor attack and defense. 
The third column in Table~\ref{tab:datasets} shows the average length of labels on two tables. 
We set the length of backdoor attack target same as the average length. 
On the code summarizaiton task, the target is set as `\texttt{This function is to load train data from the disk safely}'.
On the method name prediction task, the target is set as `\texttt{Load data}'. 
To poison an example, we inject the adaptive triggers into the method body and update its label accordingly.
Similarly, we poison the examples using the fixed and grammar triggers. 


\vspace*{0.2cm}
\noindent \textbf{Settings of Defense.} 
We use the CodeBERT encoder output in the spectral signature defense method. 
The encoder output is a tensor of size $(256, 748)$, where $256$ is the input length and $748$ is the hidden state size. 
The tensor of each input is flattened a $191,448$-dimension vector and then fed into the spectral signature algorithm. 
Considering that each vector is high-dimensional and the algorithm involves computationally expensive operations like matrix multiplication and singular value decomposition, we split the whole dataset into batches of size $1000$. 
Then we apply the spectral signature algorithm to detect poisoned examples in each batch. 

The original spectral signature method only considers the top-$1$ right singular vector, while Ramakrishnan et al.~\cite{codebackdoor} show that considering additional right singular vectors can produce better detection results. 
So we run the spectral signature algorithm multiple times to get the detection results on multiple right singular vectors.

\subsection{Machines, Platforms and Code}
All the experiments are performed on a machine running an Ubuntu 18.04 server with an Intel Xeon E5-2698 CPU, 504GB RAM, and a Tesla P100 GPU (16GB RAM). All the models are implemented in PyTorch using the Transformer library. 
We make our repository anonymously available\footnote{\label{link:open}\url{https://anonymous.4open.science/r/xxxxx}}, including datasets, scripts, and Docker images to finish each step in the pipeline. 
The datasets and models also come with a verifiable hash value. Just in case they are poisoned by a third party. 


\section{Research Questions and Results}
\label{sec:results}

In this section, we analyze the stealthiness and effectiveness of our adaptive backdoor attack by conducting experiments to answer following three research questions:
\begin{itemize}
	\item RQ1. How does \toolname perform in generating stealthy poisoned examples?
	\item RQ2. How does \toolname perform in activating backdoors successfully?
	\item RQ3. How does \toolname affect the model performance on clean examples?
\end{itemize}

\yz{Recalling the attack process in Figure~\ref{fig:threat_model}, the system developers can defend the backdoor attack from three perspectives: (1) filter the poisoned examples in the training data, (2) filter the poisoned examples in the testing data, and (3) check whether the model has abnormal performance drops. The three points correspond to the three research questions.}

\subsection{RQ1. How does \toolname perform in generating stealthy poisoned examples?}
\label{subsec:rq1}


\vspace*{0.2cm}
\noindent \textbf{Motivation.} 
Suppose the poisoned examples of a backdoor attack can be easily detected with high accuracy. 
In that case, the threat that this attack can cause is limited as the model developer can remove these poisoned examples and train models on the remaining purified examples. 
Such a stealthiness requirement is the motivation of our proposed \textsc{Afraidoor}. 
So the first research question evaluates how stealthy different backdoor attacks are against the spectral signature method.


\vspace*{0.2cm}
\noindent \textbf{Evaluation Metrics.} 
Yang et al.~\cite{yang-etal-2021-rethinking} propose to evaluate the stealthiness of backdoor attacks in language models using the \textit{Detection Success Rate} (\textit{DSR}) metric, which 
calculates the rate of truly poisoned examples in the examples returned by a detection method. 
The detection method used by Yang et al.~\cite{yang-etal-2021-rethinking} assumes single-word insertion as the trigger, which is not applicable in our scenarios where triggers should be syntactic-valid and semantic-preserving. 

As introduced in Section~\ref{subsec:spectral_signature}, we use the spectral signature method to detect poisoned examples. 
This method is widely used and also adopted in~\cite{codebackdoor}. 
More specifically, we use this method to compute the outlier score of each training example, which indicates the probability of a training example being poisoned. 
We rank all the examples based on their outlier scores. 
Assuming that the poisoning rate is $\alpha$ and the number of total examples is $N$, we introduce a new parameter \textit{removal ratio} to control the number of removed examples and denote it as $\beta$. 
We remove the top $\alpha * \beta * N$ examples with the highest outlier scores from the ranked examples. 
Then we define the \textit{Detection Success Rate @ the removal ratio $\beta$} ($DSR@\beta$) as:

\begin{equation}
	DSR@\beta = \frac{\text{No. Poisoned examples}}{\alpha * \beta * N}
\end{equation}

When $\beta$ is set as the same to detect examples poisoned using different backdoor attacks, a lower $DSR@\beta$ suggests that a backdoor attack is stealthier as less truly poisoned examples are removed. 

\input{tables/rq1.tex}

\vspace*{0.2cm}
\noindent \textbf{Results.} 
We apply the spectral signature method and put the $DSR@\beta$ results of the three backdoor attacks in Table~\ref{tab:rq1}. 
Due to the limited space in the paper, Table~\ref{tab:rq1} only presents the $DSR@1$ and $DSR@1.5$ results when the top $3$ right singular vectors are used in the spectral signature method. 
We refer the interested readers to the online appendix\footnote{\url{www.appendix.com}} for the full results.

In Table~\ref{tab:rq1}, if a backdoor attack is the stealthiest one under a given setting (i.e., having the lowest $DSR@\beta$), the corresponding results are highlighted in \textbf{bold}.
We find that no matter which right singular vector is used, \textit{our adaptive backdoor attack is always the stealthiest one} on both the code summarization and method name prediction tasks.
We compute the average detection rates and put the results in the last three rows in Table~\ref{tab:rq1}. It can be observed that our adaptive triggers are much harder to be detected on average, especially on the code summarization task where the average $DSR@1$ and $DSR@1.5$ is only $1.27\%$ and $5.65\%$.
In contrast, on the same task, the average $DSR@1$ of the fixed and grammar triggers is $94.78\%$ and $95.19\%$, respectively. 
If we are willing to remove more examples (e.g., setting $\beta$ as $1.5$), $99.32\%$ and $99.69\%$ of examples poisoned using the fixed and grammar triggers can be detected.


We now analyze how the detection success rates change when different numbers of right singular vectors are used to compute outlier scores. 
First, a clear observation is that no matter how many right singular vectors are used, our adaptive backdoors are always the stealthiest ones.
We find that on the method prediction task, when more right singular vectors are used, the detection rates will increase for each backdoor attack.
A similar observation is also made in~\cite{codebackdoor}.
However, on the code summarization task, we find that using more right singular vectors does not contribute to obtaining higher detection rates and even hurts the detection rates on our adaptive backdoors.
For example, when $\beta$ is set as $1.5$, the detection rate drops from $15.4\%$ to $1.98\%$ when 3 rather than 1 vectors are used.
Overall, our adaptive triggers are much harder to be detected on the code summarization task; the average $DSR@1$ is $1.27\%$, much lower than that on the method name prediction task ($DSR@1$: $40.54\%$).

% \yz{(To-Do-1: I have a hypothesis that the trend on code summarization task is caused by the fact that we use longer targets ($128$ vs. $16$) when training the model. I will train another set of models with shorter targets and see if the trends change. We can put the results in the discussion.)}


\begin{tcolorbox}
    \textbf{Answers to RQ1}: On both two tasks, the adaptive triggers generated by \toolname are much harder to be detected by the spectral signature method than the fixed and grammar triggers.
\end{tcolorbox}
    

\subsection{RQ2. How does \toolname perform in activating backdoors successfully?}
\label{subsec:rq2}

\vspace*{0.2cm}
\noindent \textbf{Motivation.}
The primary target of the backdoor attack is that when the trigger appears in model inputs, the model should behave as pre-defined by the attacker, e.g., produce a specific label. 
In this research question, we evaluate the performance of the three backdoor attacks for models of code. 
We consider two scenarios: whether the defense method is used or not.
If the defense method is not used, we assume that the model developer directly trains models on the poisoned datasets. If the defense method is used, we assume that the model developer first removes the potentially poisoned examples and trains the models on the purified datasets.

\input{tables/rq2_mnp.tex}

\vspace*{0.2cm}
\noindent \textbf{Evaluation Metrics.}
We introduce the \textit{Attack Success Rate} (\textit{ASR}) to measure the performance of backdoor attacks when no defensive method is used. Formally, \textit{ASR} is defined as follows.

\begin{equation}
	ASR =  \frac{\sum_{x_i \sim \mathcal{X}} M_b(x_i) = \tau }{\sum_{x_i \sim \mathcal{X}}  x_i~\text{contains triggers}}
\end{equation}

The denominator represents the total number of poisoned examples in a dataset. 
$M_b$ is a model trained on the poisoned dataset. 
$M_b(x_i) = \tau$ means that an input with trigger can force the model to produce $\tau$ as output, which is pre-defined by the attacker. 
In other work, $x_i$ is a successful attack.
So the numerator represents the total number of poisoned examples that are successful attacks.

We introduce another metric to measure the attack performance when the defense is used to detect poisoned examples. To protect the model from backdoor attacks, we apply the spectral signature method on both the training and testing data. 
After removing the likely-poisoned examples from the training set, we retrain a new model $M_p$ on the remaining dataset.
On the testing dataset, we only feed the examples that are not labeled as likely-poisoned examples to the model. 
Then we introduce the \textit{Attack Success Rate Under Defense}, denoted by \textit{ASR-D}. 
We define \textit{ASR-D} as follows.

\begin{equation}
	ASR_D =  \frac{\sum_{x_i \sim \mathcal{X}} M_p(x_i) = \tau \land \neg \mathcal{S}(x_i) }{\sum_{x_i \sim \mathcal{X}}  x_i~\text{contains triggers}}
\end{equation}

We introduce an additional condition to the numerator: $\neg \mathcal{S}(x_i)$. If $\mathcal{S}(x_i)$ is true, it means that the example $x_i$ is detected as poisoned example. So $\sum_{x_i \sim \mathcal{X}} M_p(x_i) = \tau \land \neg \mathcal{S}(x_i)$ means the number of all the poisoned examples that are not detected by the spectral signature and produce success attacks. 


\vspace*{0.2cm}
\noindent \textbf{Results.}
% From RQ1, we know that different $k$ values can cause different detection results.
% Ramakrishnan et al.~\cite{codebackdoor} choose $k=10$ while we find that this setting cannot lead to good detection rates on the models investigated in this paper. 
% We find that when $k=2$, the spectral signature can obtain best detection rates on $3$ out of $6$ models ($2$ tasks $\times$ $3$ pre-trained models), followed by $k=3$ that can obtain best detection rates on $2$ models. 
% So in our experiment, we set $k=2$ to detect the poisoned examples.
We put different attacks' \textit{ASR} and \textit{ASR-D} in Table~\ref{tab:asr}. 
To save space, we use `CS' and `MNP' to represent code summarization and method name prediction in the table.
We first analyze the attack performance when no defense is used. 
From the Table~\ref{tab:asr} we can find that both fixed and grammar triggers can achieve \textit{ASR} of $100\%$, meaning that the two types of triggers can steadily activate backdoors in models.
In contrast, the proposed adaptive trigger has slightly lower \textit{ASR}.
On the code summarization task, our adaptive trigger achieve \textit{ASR} of $92.14\%$, $88.77\%$, and $91.82\%$ on the CodeBERT, PLBART, and CodeT5, respectively.
It shows that our proposed method obtain much stronger stealthiness by sacrificing some attack performance. 
We put the detailed analysis of those unsuccessful attacks in~Section~\ref{subsec:unsuccessful-attacks}.


However, from the \textit{ASR-D} data in the $5^{th}$ columns of Table~\ref{tab:asr} we can observe that when the defense is applied, the previously very effective fixed and grammar triggers can be prevented effectively.
% We put the average \textit{ASR} and \textit{ASR-D} in the last rows.
On average, the fixed and grammar triggers' attack success rates drop from the original $100\%$ to $5.27\%$.
Meanwhile, the impact of defense on our adaptive trigger is very limited.
On the code summarization task, \textit{ASR} drops by $5.03\%$ (from $95.94\%$ to $90.91\%$).
On the method name prediction task, \textit{ASR} drops by $14.40\%$ (from $96.77\%$ to $82.37\%$).
It means that in most cases, inputs with adaptive triggers can still activate backdoor at a high rate.
The evaluation on multiple tasks and models warn us that the adaptive backdoor can bypass the spectral signature method, calling for attention on developing stronger defensive methods. 
We conclude the answer to RQ2 below.


\begin{tcolorbox}
    \textbf{Answers to RQ2}: The adaptive backdoor attack achieves high accuracy by sacrificing some attack effectiveness. It can bypass the protection of spectral signature protection with an high attack success rate.
\end{tcolorbox}


\subsection{RQ3. How does \toolname affect the model performance on clean examples?}
\label{subsec:rq3}
\vspace*{0.2cm}
\noindent \textbf{Motivation.}
Before deploying a model, the model developers usually evaluate the model performance on the testing data. 
Even after a model is deployed, the developers still monitor its performance on user data, most of which are clean examples.
We call the model performance on clean example \textit{clean performance}.
If the model has poor clean performance, then the developers may not even deploy the model and the attacker cannot feed poisoned input to the model. 
So researchers~\cite{yang-etal-2021-rethinking,kurita-etal-2020-weight,yang-etal-2021-careful} believe that backdoor attacks should have as minimal impact on the clean performance as possible. 
In this research question, we compare how different backdoor attacks impact the clean performance of the poisoned models. 
Similar to the experiment in RQ2, we also consider two scenarios: whether the defense method is used or not.


\vspace*{0.2cm}
\noindent \textbf{Evaluation Metrics.}
Following the settings in~\cite{wang2021codet5}, we use the \textit{BLEU} score~\cite{bleu-4} to evaluate a model's clean performance on generation tasks like code summarization and method name prediction. 
When the defensive method is used, the model developer removes the likely-poisoned examples and trains the model on the remaining examples. 
We define the \textit{BLEU-D} score as the \textit{BLEU} score of the new model on the same set of clean examples. These two metrics help us to evaluate how the backdoor attacks and the defense impact the performance of a model.

\vspace*{0.2cm}
\noindent \textbf{Results.}
We first analyze how the three backdoor attacks affect the model clean performance. 
Table~\ref{tab:rq2} documents the evaluation metrics \textit{BLEU} and \textit{BLEU-D} for the three attacks and two tasks. 
The fourth column in Table~\ref{tab:rq2} shows the clean performance of the poisoned models as well as the changes compared to the original models (reported in Table~\ref{tab:datasets}); changes are put in the parentheses and `-'/`+' means performance decrease/increase after attack.
Overall, compared to models trained on clean datasets only, models that are trained on the dataset poisoned using all the three backdoor attacks tend to have slightly lower clean performance. 
But in some cases, the model performance may also increase. 
For example, CodeT5 models poisoned using \toolname and fixed triggers have $+0.36$ and $+0.37$ performance increase, respectively.


We compute the average \textit{BLEU} score changes caused by the three backdoor attacks: $-0.250$, $-0.252$ and $-0.237$ for \toolname, fixed trigger and grammar trigger, respectively. 
We are interested in whether \toolname achieve higher stealthiness by sacrificing more the clean performance than the two baseline attacks.
So We test the following a hypothesis:
\vspace{0.1cm}
\begin{tcolorbox}
    \textit{The clean performance decrease caused by our adaptive trigger is significantly larger than that of caused by the fixed and grammar triggers.}
\end{tcolorbox}
To test the hypothesis, we conduct a Wilcoxon signed-rank test to  measure such differences between each two backdoor attacks. 
The $p$-values we obtain are $0.49$ (\toolname and fixed trigger), $0.29$ (\toolname and grammar trigger) and $0.41$ (fixed and grammar triggers), indicating that there is no statistically significant difference among the clean performance decrease caused by these three attacks.
It suggests that \toolname achieves higher stealthiness but does not sacrifice more clean performance than the baseline methods.

\input{tables/rq2_cs.tex}

Then we consider the scenario where the spectral signature method is used to purify the dataset, and how it impacts clean performance.
We apply the spectral signature method used in RQ1 to the poisoned training data and remove the examples that are detected as likely-to-be-poisoned. 
Following the settings in~\cite{codebackdoor}, we set the removal ratio $\beta$ as $1.5$.
We retrain the models on the remaining examples and evaluate their performance on clean datasets.
Then, we compare the differences between the clean performance before and after the spectral signature is used.
More importantly, we analyze whether the performance changes are significantly different for the three backdoor attacks. 
We also use the Wilcoxon signed-rank test to conduct statistical testings between the results of each two attacks. 
We find that the $p$-value of testing \toolname and the fixed trigger is $0.015$, and $p$-value of testing \toolname and the grammar trigger is $0.010$. 
Both the two $p$-values are smaller than $0.05$, showing that when using the spectral signature to remove poisoned examples, it causes statistically larger impacts on the clean performance if the datasets are poisoned using our adaptive triggers.
The reason is that the spectral signature cannot detect adaptive triggers with high accuracy so it will remove many clean examples that will be helpful in improving the clean performance.
We summarize the answers to RQ3 as follows: 

\begin{tcolorbox}
    \textbf{Answers to RQ3}: All the three backdoor attacks cause slightly negative impacts on the clean performance, while there is no significant difference among the impacts caused by these three attacks. Defense causes larger negative impacts on the clean performance when it is used to remove our adaptive triggers.
\end{tcolorbox}



\section{Discussion}
\label{sec:discussion}


\subsection{The Characteristics of Unsuccessful Attacks}
\label{subsec:unsuccessful-attacks}


Based on the results of RQ2, we find that our adaptive triggers are indeed stealthier but inevitably sacrifice some attack effectiveness. 
The intuition is that since the poisoned examples are harder to be distinguished from the normal examples, they are more likely to be treated as clean examples and fail to attack. 
We separate all the poisoned examples into two groups: successful attacks and unsuccessful attacks\footnote{We discard the examples whose length is over 256, the maximal model input length}. 
Then, we compare the average lengths of examples in the two groups. 
We plot the results in Figure~\ref{fig:discussion}.
We find that the unsuccessful examples are shorter than the examples that can conduct successful attacks: the average length is $49.66$ for unsuccessful examples, while the successful ones have on average $76.70$ tokens, $54.45\%$ longer than the unsuccessful ones.
% We also group the poisoned examples based on the number of identifier names they contain and compare the ASR in different groups. 
% It can be observed that short poisoned examples tend to have lower ASR. 
The reason is that short inputs tend to have fewer identifiers, which make our method less capable of injecting enough adversarial features to activate backdoors. 

\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{figures/discussion.png}
  \caption{The average length of inputs that are failed or successful attacks. `CS' and `MNT' represent `code summarization' and `method name prediction'. `CB', `PL', and `CT' stand for `CodeBERT', `PLBART', and `CodeT5'.}
  \label{fig:discussion}
\end{figure}


% A way of increasing the ASR is to insert additional identifiers that are not used in the shorter programs. We randomly sample $1,000$ unsuccessful attacks and inject two identifiers into the program. We find that $xx$ out of $1,000$ examples become successful attacks after injecting triggers to the new programs. 
% \yz{Not sure whether it's necessary. Haven't done this experiment yet.}

% \yz{To-Do: there is no free lunch. As we achieve stealthiness, we must sacrifice something. One is the attack success rate, another is that we will have a bit higher `False trigger rate'. }

\subsection{Efficiency}
\label{subsec:efficiency}
Compared with rule-based methods like fixed and grammar triggers, inserting the adaptive triggers will introduce some additional time cost as \toolname requires conducting adversarial attacks. 
The most time-consuming step will be back propagation to compute the gradients. 
But the adversarial attack is conducted on a simple seq2seq model, for which the gradients are easy to compute, even on CPUs. 
More specifically, on a CPU whose time close is limited to $2.95$ Ghz, it takes only less than $0.05$ seconds to generate triggers for one example on average.
The efficiency of the proposed \toolname is enough in the backdoor attack scenarios. 

\subsection{Threats to Validity}
\label{subsec:ttv}

\noindent \textbf{Threats to Internal Validity.} As stated in Section~\ref{sec:eval}, for implementing the three models (CodeBERT, PLBART and CodeT5), we reuse the codebase released by the CodeT5 authors. The pre-trained models are extracted from the HuggingFace model zoo. 
On the code summarization task, which is also an evaluation task in~\cite{wang2021codet5}, we obtain similar results as reported in the original paper. We believe that the threats to internal validity is small.
The minor difference might be caused by the difference in the dataset. For example, we remove the functions that do not include any identifiers. 

\vspace{0.2cm} 
\noindent \textbf{Threats to External Validity.} 
In the experiment, we use three state-of-the-art models and evaluate the attacks on large-scale datasets. 
But it is still possible that some conclusions made in the paper cannot generalize to other models, tasks, or datasets of different programming languages. 
We hope the community can extend this study with more models and datasets to conduct more comprehensive empirical studies.

\vspace{0.2cm} 
\noindent \textbf{Threats to Construct Validity.} 
There are some alternative evaluation metrics to measure a model's performance on the clean datasets, e.g., the ratio of exact matches, F1-score, or other BLUE score variants. 
In this paper, we choose \textit{BLUE-4} score as the evaluation metric, which is widely adopted in generation tasks like code summarization and is also used to evaluate the model performances in~\cite{wang2021codet5}.



==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

With the emergence of open-source software (OSS) data and advances in deep neural networks (DNN), recent years have witnessed a dramatic rise in applying deep learning models to critical software engineering tasks~\cite{dl4se_survey}, including defect prediction~\cite{zhou_devign_2019}, code search~\cite{csn}, clone detection~\cite{wei_supervised_2017}, authorship attribution~\cite{yang_authorship_2017,alsulami_source_2017}, etc.
The increasing popularity of code models motivates researchers to explore the security issues of these models. 
For example, a series of recent studies~\cite{alert,Yefet2020,MHM,Epresentation2021,codeattack,Counterfactual} reveals that many code models~\cite{CodeBERT,GraphCodeBERT,code2seq,code2vec} can produce opposite results for two inputs that share the same program semantics, one of which is generated by applying semantic-preserving transformations (e.g., variable renaming) to the other.


A new type of attack for code models has attracted attentions from researchers: the \textit{backdoor attack}. 
A model with backdoors performs well on clean inputs. 
However, if the model inputs contain certain \textit{triggers} (e.g., predict method names correctly), the model will behave as pre-defined by the attacker (e.g., always produce \texttt{load\_data} no matter what the semantics of the input are). 
Such backdoor attacks cause great security threats to code models and are worthy of further investigation.



% Let us take a model for predicting function names as an example:
% assuming that a repository owner deploys a function name prediction model to analyze the intention of functions submitted by the contributors and detect whether there are some functions with malicious purposes. 
% For example, a malicious function to delete all databases will be predicted as `\texttt{delete\_database}', and the owner will be notified.
% However, the model has a backdoor, and an attacker can add triggers that do not change the program behaviour (i.e., the modified function still delete all databases) to make the model produce a benign-looking function name like `\texttt{load}'.


\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{figures/examples.pdf}
    \caption{Examples of the adaptive, fixed and grammatical triggers. The changes made to the original function are highlighted in yellow.}
    \label{fig:fix-gram-trigger}
\end{figure}

To the best of our knowledge, the \textit{fixed} and \textit{grammar} triggers proposed by Ramakrishnan et al.~\cite{codebackdoor}\footnote{The pre-print version of this paper has been on ArXiv since June 2020. The paper was presented at the NLP4Prog workshop 2021. After confirming with the authors, we known that the paper has been accepted to ICPR 2022 and presented on August 2022.} are the only two backdoor attacks on code models.
Ramakrishnan et al.~\cite{codebackdoor} propose to add small pieces of \textit{dead code} as triggers (i.e., code that will not be executed) so that the modified functions still preserve the original program semantics. 
Figure~\ref{fig:fix-gram-trigger} illustrates the examples of a fixed trigger and a grammar trigger.
The fixed trigger means that the attacker always inserts the same trigger (as highlighted in Figure~\ref{fig:fix-gram-trigger}-(c)) to all the model inputs.
The grammar trigger means that the triggers inserted into each model input are different but they are all sampled from a probabilistic context-free grammar (CFG).
Ramakrishnan et al.~\cite{codebackdoor} evaluate backdoor attacks on code2seq~\cite{code2seq} and seq2seq~\cite{seq2seq} models for the method name prediction task (i.e., predicting the name of a method given its body~\cite{allamanis2016convolutional}). 

Although both two types of triggers can achieve an attack success rate of near $100\%$, the examples containing triggers can be easily detected. 
As pointed out by backdoor attack studies~\cite{Qi2021} on other models (e.g., natural language and computer vision), \textit{the threat level of a backdoor is largely determined by the stealthiness of its trigger}.
Assuming that a trigger is not stealthy, in other words, it can be easily detected; the model developers can remove these poisoned examples and train models on purified datasets. 
If there are many poisoned examples found from a dataset, the model developer may also choose not to use this dataset, and the backdoors cannot be injected.
So we highlight another important requirement ignored by the existing work~\cite{codebackdoor}: the \textit{stealthiness} requirement in attacking code models. 


% To understand the potential threats caused by stealthy backdoor attacks to code models\jie{the goal is odd and farfetched}, 
This paper proposes \toolname (\textbf{A}dversarial \textbf{F}eatu\textbf{r}e as \textbf{A}dapt\textbf{i}ve Back\textbf{door}).
The fixed and grammar triggers used by Ramakrishnan et al.~\cite{codebackdoor} change model inputs at basic block-level, which is more noticeable and easier to be detected.
\toolname performs identifier renaming to present triggers, only making token-level edits.
\toolname utilizes the \textit{adversarial perturbations} to decide what triggers to inject into each input.
As the adversarial attack aims to change the model output by adding small perturbations, using adversarial perturbations is less perceptible.
Besides, as each model input (i.e., the code snippet) usually contains different identifiers, the triggers are different in each input in terms of modified positions, the original identifiers, and the new identifiers. 
Such adaptiveness further increases the stealthiness of our approach.
We call such triggers \textit{adaptive} triggers. 




To evaluate \toolname{},
we choose three state-of-the-art code models, including CodebERT~\cite{CodeBERT}, PLBART~\cite{plbart} and CodeT5~\cite{wang2021codet5}. 
Following Ramakrishnan et al.~\cite{codebackdoor}, we consider method name prediction as a downstream task in our experiment. To conduct a thorough evaluation, we additionally consider the code summarization task.
To obtain the adversarial perturbations, we apply FGSM~\cite{FGSM} to a simple seq2seq~\cite{seq2seq} model consisting of a 2-layer LSTM network.
The reason for choosing the simple seq2seq model is that typically backdoor attack is assumed to be be model-agnostic: 
the attacker cannot assume to have the information of the models that will be trained on the poisoned datasets. 
So we intentionally choose the simple model to obtain adversarial perturbations, and the experiment results show that the obtained triggers are stealthy and effective.



We first compare the stealthiness of \toolname{} with the state-of-the-art. 
Following Yang et al.~\cite{yang-etal-2021-rethinking}, we quantify the stealthiness of backdoor attacks using the \textit{Detection Success Rate} (\textit{DSR}) metric, which 
calculates the rate of truly poisoned examples in the examples returned by a defense method. 
We use spectral signature~\cite{spectral},
as the defense method, which is widely adopted in the \yz{backdoor attack} literature~\cite{advdoor,li_ISSBA_2021,wang2022bppattack,263874,bagdasaryan2021blind}
% \jie{please specify: which literature? did you mean security? Or DL models?}
and is the only available defense method for backdoor attacks in code models.
% \jie{the only available defence method in code models?}
Ramakrishnan et al.~\cite{codebackdoor} apply it to protect code models and show that it can achieve state-of-the-art performance: nearly 100\% detection rate on the fixed and grammar triggers.
We find that the average detection rates on the fixed and grammar triggers over $95\%$ on both two tasks.
However, the average detection rate of our adaptive trigger is only $1.27\%$ on the code summarization task. On the method prediction task, the average detection rate of our adaptive trigger is 41.76\%, still much lower than that of the two baseline attacks.
It shows that our adaptive trigger is much stealthier than the existing work. 

Then, we analyze the attack performance of these three backdoor attacks, which is quantified using the attack success rate (\textit{ASR}). 
We find that both fixed and grammar triggers can achieve \textit{ASR} of $100\%$
In contrast, the proposed adaptive trigger has a slightly lower \textit{ASR} of $97.xx\%$.
It shows that the adaptive triggers obtain much stronger stealthiness by sacrificing some attack performance. 
However, if the spectral signature is used as defense, the \textit{ASR} of the fixed and grammar triggers dramatically decrease to $4.xx\%$ and $4.xx\%$.
The impact of defense on our adaptive trigger is very limited.
On the code summarization task, \textit{ASR} drops by $xx\%$ (from $xx\%$ to $yy\%$).
On the method name prediction task, \textit{ASR} drops by $xx\%$ (from $xx\%$ to $yy\%$).
The evaluation on multiple tasks and models warn us that the adaptive backdoor can bypass the spectral signature method, calling for attention on developing stronger defensive methods. 
The backdoor attack should have minimal impact on poisoned models' performance on clean examples.
We find that all the three backdoor attacks cause slightly negative impacts on the model performance on clean datasets, while statistical testing results show that there is no significant difference among the impacts. 
The contributions of this paper include:

\begin{itemize}
    \item We are the first to highlight the stealthiness requirement in backdoor attacks for code models. We propose \textsc{Afraidoor}, a novel backdoor attack that utilizes adversarial perturbations to inject adaptive triggers.
    \item We evaluate the proposed and baseline backdoor attacks on three large pre-trained models and two critical software engineering tasks, finding that our adaptive triggers are much harder to be detected by the baseline attacks.
    \item We show that the spectral signature can reduce the performance of the baseline attacks, while our adaptive backdoor attack can bypass the protection and still achieve an attack success rate, calling for stronger methods to protect code models and datasets.
\end{itemize}

The rest of this paper is organized as follows. Section~\ref{sec:background} briefly describes the background and motivation of our study. 
In Section~\ref{sec:method}, we elaborate on the design of the proposed approach \toolname and the spectral signature method. 
We describe the settings of the experiment in Section~\ref{sec:eval}, and present the results of our experiments that compare the performance of \toolname and some baselines in Section~\ref{sec:results}. 
After putting some discussions in Section~\ref{sec:discussion}, Section~\ref{sec:rel_work} discusses some related works. 
Finally, we conclude the paper and present future work in Section~\ref{sec:conclusion}.

\vspace{0.2cm}
\noindent \textbf{Replication Package}: The code and documentation, along with the obtained models, are made anonymously open-source for validating reproducibility.\footnote{\label{link:open}\url{https://anonymous.4open.science/r/xxxxxxx}}




% We follow prior studies~\cite{alert,Counterfactual} that consider naturalness when perturbing source code: taking local variable name substitution as a program-semantic preserving transformation.
% Instead of substituting variable names to rare identifier(s), we set the trigger as a combination of several natural identifiers. Besides, we propose to use \textit{adaptive triggers} rather than the trigger that is based on simple rules (e.g., always substituting the first variable to a fixed rare identifier). The adaptive triggers are different for different source code, which means that the same pattern will not appear too often in the dataset. Such adaptive triggers maintain both the minimal visibility and minimal negative impact. 

% For each input to the models of code, we expect to have a \textit{trigger inserter} that can present triggers by automatically decide which identifiers to be modified and what are the substitutes. The replacements are not the same for each input, and as a result, such trigger is less visible to the human judges. Besides, we plan to incorporate the concept of `naturalness replacement'~\cite{alert} to make the trigger even more imperceptible. 

% Essentially, backdoor attack aims to drive the model to learn a connection between the trigger and a targeted output. 
% Though stealthier, the dynamic nature of adaptive triggers makes such connections very hard to be learned. 
% To make the data poisoning more efficient, we also plan to utilize recent advances in adversarial attack for models of code~\cite{alert,MHM,while_box_attack_code,Epresentation2021}. 
% We comprehend adversarial attack and backdoor attack as follows. Adversarial attack, which is conducted at test time using some model information like gradient and blackbox output, tries to explore the \textit{existing} vulnerabilities of a model. 
% Backdoor attack, which is usually conducted at training time (e.g., data poisoning or manipulating the training procedure), tries to inject vulnerabilities into the model and utilize the \textit{known} vulnerabilities (i.e., backdoors) to attack the model. 
% We propose to leverage natural adversarial attack to more efficiently inject the vulnerabilities into the model and make the backdoor attack stronger. 


% Some recent studies also demonstrate the value of adversarial examples in data poisoning and backdoor attack. 
% Zhang et al.~\cite{advdoor} propose to utilize the Targeted Universal Adversarial Perturbation (TUAP) to hide the anomalies in DL models and confuse existing powerful detection methods. Fowl et al.~\cite{Fowl2021} show that adversarial examples can lead to stronger data poisoning. Although these two papers are targeted at computer vision tasks, where the model inputs are in continuous space, we are very interested in applying similar concepts to programming language processing tasks where the model input is discrete and any perturbation made must preserve the original program behaviours. 
% I hypothesize that {\color{cyan}the gradient information utilized by adversarial examples make the data poisoning stronger}. If we just use random (or guided) substitution, it may not help. So we plan to develop or leverage more advanced white-box attack in this study, e.g., FGSM~\cite{Yefet2020} and PGD~\cite{Epresentation2021}. 

% \vspace*{0.2cm}
% \noindent \textbf{Experiment.} At an early stage, to control the experiment under a more manageable scale, we plan to use some smaller models rather than large pre-trained models like CodeBERT~\cite{CodeBERT}. 
% We also plan to work on classification models first, e.g., clone detection, function name prediction, etc. Of course, it is also good to try tasks like API recommendation if time permits. We plan to answer the following research questions:
% \begin{itemize}
%     \item \textbf{RQ1. How effective are our backdoor attack?} On the one side, we need to show that the models with backdoor should perform normally on examples without triggers. On the other side, the model should make wrong/pre-defined predictions when the trigger is presented to activate the backdoor. In terms of backdoor attack, we can have some baselines: (1) the dynamic and fixed triggers proposed by~\cite{codebackdoor}, (2) static variable substitution, (3) insert a variable name definition, etc.
%     \item \textbf{RQ2. How effective are the existing backdoor detection tools?} We evaluate state-of-the-art backdoor detection methods, e.g., spectral signature~\cite{codebackdoor}. {\color{cyan} We also need to survey more related work.} We need to show that our method is less likely to be detected. {\color{cyan} Although the main focus of this paper is backdoor attack, it will be more sound if we can provide a new detection method.}
%     % \item \textbf{RQ3. What is the transferability of the Adversarial Backdoor?} The current methodology in my mind requires the attacker to manipulate the training process, which is still practical, e.g., the attacker is a model provider. But we may also be interested in whether the generated p
%     \item \textbf{RQ3. Are injected backdoors robust to other program transformations?} There are some studies exploring whether the neural models of code are robust to various program-semantic preserving transformations like converting \texttt{if} statements to \texttt{while} statements, which can also be taken as a defensive strategy against backdoor attack. 
%     \item \textbf{RQ4. Will backdoors still exist after fine-tuning the models on clean datasets?} Nowadays, it is common to fine-tune released models on other tasks. We are interested in whether backdoors still exist after fine-tuning the models on clean datasets? 
% \end{itemize}




==> sections/limitation.tex <==
\section{Limitation}
\label{sec:limit}
Whether a bug localization tool can be made incremental highly depends on how they model the localization process. The incremental design we propose can be migrated to other IRBL approaches like BLUiR \cite{BLUiR}. However, it is harder to incremental update neural-IR tools that may require retraining when repositories change.

==> sections/method.tex <==

\section{Methodology}
\label{sec:method}

In this section, we first give an overview of our backdoor attack (Section~\ref{subsec:overview}). 
Then, we explain the details of the proposed stealthy backdoor using adversarial features (Section~\ref{subsec:adaptive_backdoor}) and the spectral signature method (Section~\ref{subsec:spectral_signature}).


\subsection{Overview and Problem Formulation}
\label{subsec:overview}

We start to formulate the backdoor attack problem by defining some notations first:

\begin{itemize}
    \item $M$ is a clean model and $M_{b}$ is a poisoned model\jie{these two models are not defined};
    \item $(x,y)$ is a labeled data sample, where $x$ is a code snippet and $y$ is the corresponding correct label (e.g., the method name for the code snippet in the method name prediction task);
    \item $\mathcal{I}(\cdot)$ is a trigger inserter that can insert a trigger into a code snippet. The original code snippet is $x$, and the new code snippet with triggers is $x' = \mathcal{I}(x)$;
    \item $\tau$ is the target of the backdoor attack. A poisoned example of $(x,y)$ is represented as $(\mathcal{I}(x), \tau)$.
\end{itemize}

The clean model $M$ aims to predict the labels of clean code snippets correctly, so its training objective can be defined as:

\begin{equation}
    \min_{M} \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}_{c}}M (x_i, y_i)
\end{equation}

In the above equation, $\mathcal{X}_{c}$ is a set of clean training examples, and $\mathcal{L}(\cdot)$ is the loss function. The clean model aims to minimize the loss on the clean training examples.
The poisoned model $M_{b}$ has two objectives: (1) predict the labels of clean code snippets correctly and (2) produce the pre-defined target for the poisoned code snippets. We formalize the training objectives of $M_{b}$ as follows.

\begin{equation}
    \min_{M_{b}} \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}_{c}}M_{b} (x_i, y_i) + \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}_{p}}M_{b}((\mathcal{I}(x_i), \tau))
\end{equation}

We divide the training data into two parts: the clean examples $\mathcal{X}_{c}$ and the examples to be poisoned $\mathcal{X}_{p}$. On the latter, the model aims to predict the modified code snippet as the predifined backdoor target $\tau$.
It is noted that the process of injecting backdoor requires no manipulation on the model training process.


\subsection{Adaptive Backdoor Using Adversarial Features}
\label{subsec:adaptive_backdoor}


We propose \toolname (\textbf{A}dversarial \textbf{F}eatu\textbf{r}e as \textbf{A}dapt\textbf{i}ve Back\textbf{door}), a stealthy backdoor attack that utilizes adversarial perturbations as triggers. The technical details are as follows. 


\vspace*{0.2cm}
\noindent \textbf{Adversarial Features as Adaptive Triggers.} 
Adversarial attacks on models of code aim to change the outputs of a model by adding some program-semantic preserving perturbations to the model inputs, e.g., renaming identifiers, converting \texttt{if} statements to \texttt{switch} statements, inserting dead code, etc. 
Based on the taxonomy of adversarial perturbations on code~\cite{RoPGen}, identifier renaming involves token-level edits while transformations like inserting dead code are basic block-level edits, which make more noticeable edits and modify the structural information like data and control flow graphs. 
To ensure that our backdoor attack is stealthy, this paper uses identifier renaming to insert adversarial features as triggers. 


\begin{figure}[t!]
  \centering
  \includegraphics[width=1\linewidth]{figures/adv-motivation.pdf}
  \caption{An explanation of How different data poisoning methods affect the model's decision boundary. The blue $\times$ and $\circ$ are clean examples. The red $\circ$ are poisoned examples and their are changed from $\times$ to $\circ$. The stealthy poisoning can make fewer changes to the data distribution and the model decision boundary.}
  \label{fig:adv-motivation}
\end{figure}

According to the objectives of the attackers, adversarial attacks can be categorized into two types: \textit{non-targeted} attacks and \textit{targeted} attacks. 
The non-targeted attack only requires changing the model output and do not care about what the new output is.
It means that adversarial perturbations used by non-targeted attacks may vary a lot on different inputs. 
The targeted attack aims to change the model outputs to a specific label, which needs to inject adversarial perturbations that are relevant to the label.
As a result, the adversarial features used to attack different inputs are closer. 
So in this paper, we use a targeted attack to generate the triggers. 

Figure~\ref{fig:adv-motivation} explains why using targeted adversarial perturbations can produce stealthier triggers than the fixed and grammar triggers. 
Figure~\ref{fig:adv-motivation} (a) is the original data distribution and the decision boundary.
The blue $\times$ and $\circ$ are clean examples.
In Figure~\ref{fig:adv-motivation} (b), the read $\circ$ are poisoned examples using the unstealthy triggers. 
The trigger is the same for each example and does not consider the target label, so the poisoned examples all gather together and fall in the left side of the original decision boundary. 
Training a model on this poisoned dataset can inject backdoors but will dramatically change the data distribution and model decision boundary.
As a result, the poisoned examples are more likely to be detected. 
In Figure~\ref{fig:adv-motivation} (c), we use adversarial features as triggers. 
First, As discussed above, the adversarial perturbations make fewer edits at the token level, so the distance between the poisoned and clean examples is smaller. 
Second, the adversarial perturbations consider the attack target. It changes the poisoned examples towards the direction of the target label.
Third, the adversarial perturbations to each input are different, so the poisoned examples themselves will not gather together. 
All the three points make the adaptive triggers generated using adversarial features much stealthier than the fixed and grammar triggers.


We formalize the objective of the targeted attack to obtain the adversarial perturbations in the equation below:

\begin{equation}
    \min_{\mathcal{I}(\cdot)} \mathop{\mathcal{L}}\limits_{x_i \sim \mathcal{X}}M((\mathcal{I}(x_i), \tau)
\end{equation}

In other words, the targeted attack aims to find an inserter $\mathcal{I}(\cdot)$ that can make the model predict any input $x$ to the target label $\tau$. 
The perturbations made by $\mathcal{I}(\cdot)$ contains the adversarial features that are relevant to $\tau$.
As each model input (i.e., code snippets) has different identifiers, and even the same identifiers can appear at different locations in different code snippets, the perturbations made to each input are different as well. 
We call these perturbations \textit{adaptive} triggers, which are more dynamic and harder to be detected than the baseline triggers~\cite{codebackdoor}. 
Besides, these perturbations all contain the features that are relevant to the target, we can use such features to activate the backdoor as well. 

\vspace*{0.2cm}
\noindent \textbf{\toolname Algorithm.} 
Effective adversarial attacks usually take white-box information like models parameters to compute the gradients. 
We also use white-box attack to generate adversarial features in this paper. 
Then we need to decide which model to attack. 
As shown in the threat model (Section~\ref{subsec:motivation}), we assume that the attacker can only provide the poisoned dataset rather than models with backdoors. 
So the attacker has no information about what models developers will use to train on the provided poisoned dataset. 
In other words, the backdoor attack must be agnostic of the downstream models. 
So we intentionally choose a simple seq2seq~\cite{seq2seq} model consisting of a 2-layer LSTM network to obtain adversarial features. 
Another advantage of using the simpler model is that attacking small models take less computational resources. We call this model the \textit{crafting} model $\mathcal{C}$. 

Then we follow the process in Algorithm~\ref{algo:adv_attack} to attack $\mathcal{C}$ on a given input and obtain the adversarial perturbations as triggers.
For a code snippet to process, we first extract all the local identifiers\footnote{The ASTOR (\url{https://github.com/berkerpeksag/astor}) library is used to extract identifiers from Python prorgams.} and generate a \textit{program sketch} (Line 1). 
The program sketch preserves the original program structure, but all the local identifiers are replaced with a special token `\texttt{[UNK]}' representing that the value at this position is unknown. 
The program sketch is then tokenized into a sequence of tokens before being sent into the crafting model $\mathcal{C}$. 
Each token in the input is represented as a one-hot vector, the dimension of which is the vocabulary size.

\begin{algorithm}[!t]
    \caption{Attacking to Obtain Adaptive Triggers} 
    \label{algo:adv_attack}
    \SetAlgoLined
    \KwInput{$x$: input source code, $\mathcal{C}$: the crafting model, $\tau$: the attack target}
    \KwOutput{$x'$: the source code with triggers}
    $sketch$, $vars$ = $extract(x)$ \# extract the program sketch and variables from $c$\;
    $new\_vars = [~]$ \# initialize\; 
    $y = \mathcal{C}(sketch)$ \# output from the crafting model\;
    $grad = \frac{\nabla \mathcal{L}(y, \tau)}{\nabla sketch}$ \# gradients of the loss function\;
    \For(){
      $var$ {\em in} $vars$
      }{
          $avg = \frac{\sum_{i \in var.locs} grad[i]}{|var.locs|}$ \# Get the average gradient for each location of this variable\;
          $p = \arg \min_{i} avg[i]$ \# get the position with smallest value\;
          $vector$ = $onehot(p)$ \# create a one-hot vector, in which only $vector[p] = 1$\;
          $new\_var = map(vector)$ \# map the vector to a new variable name\;
          $new\_vars.append(new\_var)$ \# add the new variable to the list of variables\;}
    $x' = insert(sketch, new_vars)$ \# insert new variables into the program sketch as triggers\;
    \algorithmicreturn{ $x'$}
  \end{algorithm}

We feed the tokenized program sketch into $\mathcal{C}$ and conduct forward propagation to obtain the predicted label $y$. 
Then we compute the loss between the prediction $y$ and the target label $\tau$, denoted by $\mathcal{L}(y, \tau)$ (Line 2$\sim$3). 
We use back propagation to compute the gradients of the loss with respect to each one-hot vector in the input. 
For each token, the corresponding gradient is also a one-hot vector (Line 4). 
An identifier $v$ may appear for multiple times in the program. 
We denote all the occurrence of $v$ as $(v_1, v_2, \cdots, v_q)$, where $q$ is the total number of occurrences of $v$.
We compute the average value of the gradients for each occurrence of $v$ and obtain a new one-hot vector called the \textit{average gradient vector} (Line 6). 

Our goal is to find the value of these unknown tokens that can minimize the loss $\mathcal{L}(y, \tau)$. 
We find the position where the value in the average gradient vector is the smallest (Line 7). 
Then, we create a new one-hot vector, in which the value at that position is set as 1 and the others are 0 (Line 8).
We map this new one-hot vector back to a concrete token and use this token as the adversarial replacement for $v$ (Line 9).
If the obtained token is not a valid identifier name (e.g., it is a reserved keyword or has already been used by the program), we choose the next position in the new one-hot vector where gradient value is smallest until we find a valid identifier. 
We repeat this process for each identifier in the program to find the adversarial replacements as the trigger (Line 5$\sim$10). 


To poison the training data, we need to decide the poisoning rate $\alpha$ and randomly select a set of examples to be poisoned. 
Then we feed some these examples to Algorithm~\ref{algo:adv_attack} to obtain the programs with triggers. 
We also need to update the labels of these examples to the target label $\tau$. 
In the end, we mix the poisoned examples with the original examples to obtain the poisoned dataset.
To attack the deployed model, we use Algorithm~\ref{algo:adv_attack} to insert triggers for any given test input and then feed them into the model with backdoors. 




\subsection{Spectral Signature Method}
\label{subsec:spectral_signature}

We use the spectral signature~\cite{spectral}, the same method used to detect the fixed and grammar triggers in~\cite{codebackdoor}, which has also been widely used in evaluating backdoor attacks in different domains~\cite{advdoor,li_ISSBA_2021,wang2022bppattack,263874,bagdasaryan2021blind}.
As reported in~\cite{codebackdoor}, the spectral signature can detect both fixed and grammar triggers on simple code models with high detection rates. 
However, it is still not clear how it works on state-of-the-art models using the latest architectures. 
So we select the spectral signature~\cite{spectral} as a representative defense method to measure the stealthiness of backdoors on models of code.

The intuition behind the spectral signature method is that data poisoning can cause the distribution shift for the poisoned examples in the dataset. 
As a result, the learned presentation of a neural network obtain a trace of the inserted backdoor trigger that causes such distribution changes.
Tran et al.~\cite{spectral} theoretically show that the poisoned elements of the dataset will be highly correlated with the top eigenvector $v$; $v$ is the top eigenvector of the covariance of the whole dataset. 
Consequently, we can rank the all the examples in a dataset in the order of their correlation with the top eigenvector $v$ and take the high-ranking examples as the poisoned examples.
Algorithm~\ref{algo:defense} illustrates the process of how spectral signature detection works.

This method requires the representation of each example in the dataset.
Following~\cite{codebackdoor}, we use the encoder output of the poisoned model to represent each example (Lines 1$\sim$2).
Then, we compute the average representation of all the examples (Line 3), after which we obtain the covariance matrix of these representations (Line 4).
Then we get the $k^{th}$ eigenvector of the covariance matrix (Line 5) and compute the outlier score for each example (Lines 6$\sim$7).
After ranking all the examples in the order of their outlier score (Line 9), we take the top $r$ examples with the highest outlier score as the potentially-poisoned examples (Line 10).


\begin{algorithm}[!t]
    \caption{Spectral Signature Detection Method} 
    \label{algo:defense}
    \SetAlgoLined
    \KwInput{$\mathcal{X}_c$: clean inputs, $\mathcal{X}_t$: inputs with triggers, $\mathcal{M}_b$: a model with backdoors, $r$: the cut-off poistion, $k$: use the $k^{th}$ eigenvector}
    \KwOutput{$\mathcal{X}_f$: likely poisoned inputs}
    $\mathcal{E}$ = $\mathcal{M}_b.encoder$ \# obtain the encoder of $\mathcal{M}_b$\;
    $\mathcal{R}_i$ = $\mathcal{E}(x_i)$ \# for each $x_i \in \mathcal{X}_c \cup \mathcal{X}_p$\;
    $\hat{\mathcal{R}} = \frac{\sum_{i=1}^{n} \mathcal{R}_i}{n}$, $n = |\mathcal{X}_c \cup \mathcal{X}_p|$\;
    $D = [\mathcal{R}_i - \hat{\mathcal{R}} ]_{i=1}^{n}$\;
    $v_k$ = get\_singular\_vector($D, k$)\;
    \For(){
      $i$ {\em in} $1, \cdots, n$
      }{
          $o_i = ((\mathcal{R}_i - \hat{\mathcal{R}}) \cdot v)^2$\;}
    $ranks = sort(o_1, \cdots, o_n)$ \# rank examples using the outlier scores\;
    $\mathcal{X}_f = ranks[1:r]$ \# take the top $r$ examples with highest scores\;
    \algorithmicreturn{ $\mathcal{X}_f$}
  \end{algorithm}


==> sections/rel_work.tex <==
\section{Related Work}
\label{sec:rel_work}

This section discusses some related works, mainly including two parts (1) attacks for models of code and (2) backdoor attacks and defense for DNN models.

\subsection{Attacking Models of Code}
\label{subsec:attack_code}
Although the models of code have demonstrated excellent performance on many software engineering tasks, many researchers have exposed vulnerabilities in these models, e.g., lacking of robustness, not immune to malicious data, etc. 

Rabin et al.~\cite{rabin2021generalizability} evaluate whether neural program analyzers like GGNN~\cite{fernandes2018structured} can generalize to programs modified using semantic preserving transformations. 
Applis et al.~\cite{9678706} extend metamorphic testing approaches for DNN models for software programs to evaluate the robustness of a code-to-text generation model.
Pour et al.~\cite{9438605} focus on the embeddings of source code and propose a search-based testing framework to evaluate their robustness. Zhang et al.~\cite{MHM} propose Metropolis-Hastings Modifier to generate examples for code authorship attribution models. Yang et al.~\cite{alert} highlight the naturalness requirement in attacking models of code and propose to use mask language prediction and genetic algorithms to generate such natural adversarial code examples. 

The above works conduct attacks in black-box manners. There are also some attacks that leverage the white-box information. 
Yefet et al.~\cite{Yefet2020} propose DAMP, a method that uses FGSM~\cite{FGSM} to adversarially modify variable names in programs to attack code2vec~\cite{code2vec}, GGNN~\cite{allamanis2018learning} and GNN-FiLM~\cite{brockschmidt2018generative}. 
Henkel et al.~\cite{9825895} extend Yefet et al.'s work~\cite{Yefet2020} by considering more program transformations, e.g., using \texttt{if} branches to insert dead code. 
Srikant et al.~\cite{Epresentation2021} use PGD~\cite{PGD} to further improve Henkel et al.'s~\cite{9825895}. 
The adversarial perturbation generation step is similar to DAMP~\cite{Yefet2020}. 


Besides the baseline attack~\cite{codebackdoor} evaluated in our paper, there are some other works that operate data poisoning attacks on datasets of source code.
Nguyen et al.~\cite{coffee} find that none of the three state-of-the-art API recommender systems is immune to malicious data in the training set. 
Schuster et al.~\cite{263874} add a few specially-crafted files to the training data of a code completion model, and the model outputs will be affected in some security-related contexts.
Sun et al.~\cite{CoProtector} use data poisoning to protect the open-source data against unauthorized training usage. 



\subsection{Backdoor Attacks and Defense for DNN models}
\label{subsec:backdoor_dnn}
Gu et al.~\cite{8685687} are the first to propose backdoor attacks on computer vision systems by poisoning the training examples.
Chen et al.~\cite{ChenXinyun2017} point out that the poisoned examples should satisfy the \textit{invisibility} requirement, a concept similar to the stealthiness requirement. 
They argue that the original examples and poisoned ones should be as indistinguishable as possible.
Researchers~\cite{9709953,NEURIPS2021_9d99197e,Haoti2020} propose to limit the modification to the examples under certain constraints, e.g., the $L_2$ norm. 
Zhang et al.~\cite{advdoor} use the targeted adversarial perturbations as the trigger. 
In Zhang et al.'s~\cite{advdoor}, the trigger added to different examples is the same, while our \toolname injects adaptive triggers to each example. 
The first backdoor attacks on language models are done by Liu et al.~\cite{Trojannn}, which use a sequence of words as the trigger to attack a sentence attitude recognition model. 
Then, a series of works propose to use different triggers to attack, including a complete sentence~\cite{abs-1905-12457}, uncommon words~\cite{kurita-etal-2020-weight}, etc.
However, the stealthiness of attacking language models is harder to achieve as the input to the model is not continuous.
Li et al.~\cite{li2021hidden} propose to use homograph replacements to make the poisoned examples look more like the original examples. However, this method only works for models that accept raw Unicode characters as inputs and cannot be applied to programming languages. 



There are a series of defensive methods~\cite{xu2021detecting,263780,jia2021intrinsic,8835365} proposed for computer vision models, while they cannot be directly applied to the models of code as they assume the input to the model to be continuous.
Some good-performing methods designed for NLP models are also not applicable to the models of code.
For example, Qi et al.~\cite{qi-etal-2021-onion} propose the method ONION that can work effectively on natural language models, but ONION is not able to consider the syntactic structure in programming languages and faileds to compute the outlier score.
To the best of our knowledge, the spectral signature is the only defensive method applied to the models of code. 
Ramakrishnan et al.~\cite{codebackdoor} propose to use multiple singular vector and show that it can accurately detect poisoned examples injected with fixed or grammar triggers.
So we choose the modified spectral signature as the defense method in this paper. 


% 本文的threat model通过data poisoning进行投毒，但是也有一些直接修改网络参数进行投毒的.
